CAST: A Correlation-based Adaptive Spectral Clustering Algorithm on Multi-scale Data

We study the problem of applying spectral clustering to cluster multi-scale data, which is data whose clusters are of various sizes and densities. Traditional spectral clustering techniques discover clusters by processing a similarity matrix that reflects the proximity of objects. For multi-scale data, distance-based similarity is not effective because objects of a sparse cluster could be far apart while those of a dense cluster have to be sufficiently close. Following [16], we solve the problem of spectral clustering on multi-scale data by integrating the concept of objects' "reachability similarity" with a given distance-based similarity to derive an objects' coefficient matrix. We propose the algorithm CAST that applies trace Lasso to regularize the coefficient matrix. We prove that the resulting coefficient matrix has the "grouping effect" and that it exhibits "sparsity". We show that these two characteristics imply very effective spectral clustering. We evaluate CAST and 10 other clustering methods on a wide range of datasets w.r.t. various measures. Experimental results show that CAST provides excellent performance and is highly robust across test cases of multi-scale data.

==> tex/algorithm_report.tex <==
\section{Algorithm}
\label{sec:algorithm}

In this section we describe our ROSC algorithm. Figure~\ref{figure:flow_graph}(c) shows a 
flow diagram of ROSC. ROSC follows the basic pipeline of spectral clustering except that
it generates a coefficient matrix $Z$ 
%(shown in the red box of the diagram) 
and feeds it
 into the clustering pipeline in place of
the similarity matrix $S$. 
The objective is to find a  $Z$ that possesses  grouping effect. 
To achieve that, ROSC uses PI to obtain {\pev}s from which a basic $Z$ is derived.
Next, it generates the TKNN graph with which $Z$ is rectified. 
In the following, we discuss how $Z$ is derived from the {\pev}s, define the TKNN graph,
describe the rectification process, 
and prove that the resulting $Z$ has the desired grouping effect. 

%
%In this section, we propose a \textbf{RO}bust \textbf{S}pectral \textbf{C}lustering method ROSC. 
%Instead of directly performing spectral clustering on the given similarity matrix, 
%it constructs a new matrix that reserves the efficacy of effective similarities 
%and rectifies ineffective ones in the raw similarity matrix.
%The new matrix will lead to a more robust spectral clustering.

\comment{
\subsection{Model overview}
The overall framework of ROSC is summarized as follows.

First, generate a set of pseudo-eigenvectors.
Since the standard spectral clustering methods using only the dominant eigenvectors may fail 
in the data containing multi-scale clusters,
we generate a set of pseudo-eigenvectors to fuse more useful cluster-separation information.

Second, rectify the given similarity matrix.
The failure of spectral clustering on multi-scale data originates from the inaccurate similarity matrix.
Therefore, we rectify the matrix and aim to achieve a new one
that can more accurately reflect the true similarities between objects.
%This is a major problem to be addressed.

Third, perform spectral clustering.
After rectification, the new similarity matrix will be more accurate and it will be safer to perform spectral clustering. 

These three steps will lead to robust clustering results and next we introduce each step in detail.
}

\subsection*{Pseudo-Eigenvectors}
\label{sec:sec:pseudo}
Given a similarity matrix $S$, we normalize it and apply PI to obtain {\pev}s.
%When dealing with multi-scale data,
%spectral clustering
%using only the top-$k$ eigenvectors may fail while some other eigenvectors may be useful~\cite{lin2010power}.
%Therefore, it is necessary to fuse the discriminative cluster-separation information in all eigenvectors
%and PI provides such fusion by returning a pseudo-eigenvector.
%However, when the number of clusters is large,
%a single pseudo-eigenvector is insufficient due to the cluster-collision problem. 
%%Since PI returns a pseudo-eigenvector that is a combination of all the eigenvectors,
Similar to~\cite{ye2016fuse},
we run PI multiple times with different random initial vectors to generate a set of {\pev}s, 
which maps each object into a low dimensional embedding.
Note that small {\ev}s are {\it shrunk} by PI~\cite{lin2010power}.
%\footnote{From Equation~\ref{eq:pi}, we see that the $i$-th 
%largest \ev\ is 
%shrunk at a rate of $\lambda_i/\lambda_1$ per iteration.}.
To alleviate the shrinkage of small {\ev}s,
we follow the approach of~\cite{huang2014diverse}
and gradually decrease the number of iterations executed in PI as more {\pev}s are obtained. 

Since the {\pev}s approximate the most dominant {\ev}, they could be similar. 
To reduce this redundancy,
whitening~\cite{kessy2017optimal} is used to make the pseudo-eigenvectors uncorrelated.
Moreover, noise in the {\pev}s are reduced 
by a rectification process, which will be discussed later.

\comment{
First, we generate a set of pseudo-eigenvectors using different random vectors $\bm{v}_0$.
From Eq.~\ref{eq:v0}, $\bm{v}_0$ can be represented by the subspace spanned by all the eigenvectors.
Suppose $\bm{e}_i$ is an informative eigenvector with a relatively small eigenvalue $\lambda_i$.
Given a $\bm{v}_0$, if it has a dominant component in the direction of $\bm{e}_i$, 
i.e., the associated coefficient $c_i$ is large, 
with an appropriate number of iterations, $c_i\lambda_i^t\approx c_2\lambda_2^t$,
the effect of $\bm{e}_i$ will be finally retained in the pseudo-eigenvector.
Therefore, multiple pseudo-eigenvectors generated by different $\bm{v}_0$
may increase the chance to hold all the informative eigenvectors.

Second, we can control the number of iterations in PI.
In PIC, the \emph{velocity} and \emph{acceleration} at the $t$-th iteration are respectively defined as
$\bm{\delta}_t = \bm{v}_t - \bm{v}_{t-1}$ and $\bm{\epsilon}_t = \bm{\delta}_t-\bm{\delta}_{t-1}$.
A threshold $\epsilon$ is introduced to measure the acceleration change in two consecutive iterations 
and stop PI when $|\bm{\epsilon}_t-\bm{\epsilon}_{t-1}|<\epsilon$.
However,
since the effect of eigenvectors corresponding to smaller eigenvalues will shrink as $t$ increases,
we can decrease the number of iterations by gradually increasing the $\epsilon$ value,
which provides another way to keep useful information in ``less important'' eigenvectors. 
}

\subsection*{Transitive {\it K} Nearest Neighbor (TKNN) Graph}

%\begin{figure}
%    \centering
%        \includegraphics[width = 0.8\linewidth]{figure/example1.eps}
%        \caption{An toy example}
%        \label{figure:example1}
%\end{figure}

%The \emph{$K$ nearest neighbor} (KNN) graph is generally used to depict the most adjacent relations between objects,
%in which the linked objects are generally assumed to share common characteristics.
%Given a set of objects $\mathcal{X} = \{\bm{x}_1,\bm{x}_2,...,\bm{x}_n\}$,
%the KNN graph $G_{K} = (V, E)$ is a graph with $V = \mathcal{X}$ and $E = \{e_{ij}\}$.
%%An edge $e_{ij}$ between $\bm{x}_i$ and $\bm{x}_j$ indicates
%%$x_j \in N_K(\bm{x}_i)$ or $x_i \in N_K(\bm{x}_j)$,
%%where $N_K(\bm{x}_i)$ denotes the set of $K$ nearest neighbors of $\bm{x}_i$.
%%at least one of the two end nodes is in the $K$ nearest neighborhood of the other.
%%However, the $K$ nearest neighborhood relation is not symmetric,
%%i.e., $x_j \in N_K(\bm{x}_i)$ is inequivalent to $x_i \in N_K(\bm{x}_j)$, 
%Some previous work~\cite{yin2016laplacian} simply considers $e_{ij}$
%exists when $\bmx_j \in N_K(\bmx_i)$ or $x_i \in N_K(\bmx_j)$,
%where $N_K(\bmx_i)$ denotes the set of $K$ nearest neighbors of $\bmx_i$.
%However,
%in the case of data containing multi-scale clusters,
%such definition may lead to an edge between
%two objects in different clusters.
%Fig.~\ref{figure:example1} shows an toy example which consists of two multi-scale clusters
%marked by ``$\times$" and ``$+$" respectively.
%For object $\bmx_1$,
%object $\bmx_2$ is its nearest neighbor.
%But for $\bmx_2$, $\bmx_1$ is far away from it.
%In this case, there will be an edge between $\bmx_1$ and $\bmx_2$ in the traditional KNN graph.
%However, since $\bmx_1$ and $\bmx_2$ belong to different clusters,
%they should not be connected.

Our objective is to capture the high correlations between objects that belong to the same cluster even 
 though the objects could be located at distant far ends of a cluster. 
 These correlations are expressed via a TKNN graph, which is used to 
 regularize the coefficient matrix $Z$.

\begin{definition}
\label{def:nei_relation}
\textbf{(Mutual  $K$-nearest neighbors)}
Let $N_K(x)$ be the set of $K$ nearest neighbors of an object $x$.
Two objects $x_i$ and $x_j$ are said to be mutual $K$-nearest neighbors of each other,
denoted by $x_i \sim x_j$, 
iff $x_i \in N_K(x_j)$ and $x_j \in N_K(x_i)$.
\hfill$\Box$
\end{definition}

%In the case of multi-scale data,
%the KNN graph is sometimes insufficient to reflect whether two objects belong to the same cluster or not.
%For example, objects $\bmx_2$ and $\bmx_3$ in Fig.~\ref{figure:example1} belong to the same cluster, 
%but they are both far away from each other.
%%objects $x_1$ and $x_2$ are in different clusters despite their closeness.
%To construct an effective KNN graph, $\bmx_2$ and $\bmx_3$
%are expected to be linked.
%Therefore,
%the reachability between two objects is introduced.

\begin{definition}
\label{def:reachability}
\textbf{(Reachability)}
Two objects $x_i$ and $x_j$ are said to be reachable from each other
if there exists a sequence of $h \geq 2$ objects 
 $\{x_i = x_{a_1}, \ldots, x_{a_h} = x_j\}$ such that
 $x_{a_r} \sim x_{a_{r+1}}$ for $1 \leq r < h$.
 \hfill$\Box$
\end{definition}

\begin{definition}
\label{def:trans_relation}
\textbf{(Transitive $K$-nearest neighbor (TKNN) graph)}
Given a set of objects $\mathcal{X} = \{x_1, x_2,..., x_n\}$,
the TKNN graph $\mathcal{G}_K = (\mathcal{X},\mathcal{E})$
is an undirected graph
where $\mathcal{X}$ is the set of vertices and $\mathcal{E}$ is the set of edges.
Specifically, the edge ($x_i$, $x_j$) $\in \mathcal{E}$
iff $x_i$ and $x_j$ are reachable from each other.
We represent the TKNN graph by an $n \times n$ {\it reachability matrix}
$\mathcal{W}$ 
whose ($i$,$j$)-entry $\mathcal{W}_{ij} = 1$ if ($x_i$, $x_j$) $\in \mathcal{E}$; 0 otherwise.
\hfill$\Box$
\end{definition}

%We note that mutual-KNN is a symmetric relation and so is reachability. 

%Compared with the traditional KNN graph, 
%the TKNN graph can more accurately reflect 
%whether two objects belong to the same cluster or not.
%It will be used in the next section to rectify the matrix of similarity between objects.
 
\subsection*{Coefficient Matrix}
%In the case of multi-scale data,
%the distance-based similarity is likely to be ineffective. 
%To improve the clustering performance,
%it is necessary to rectify the matrix.
%The rectification should follow two principles.
%First, for the effective similarities, the efficacy should be reserved.
%Second, for the ineffective ones, the efficacy should be enhanced.
%For example,
%the closeness between objects $\bmx_3$ and $\bmx_4$ in Fig.~\ref{figure:example1}
%leads to a large similarity value.
%Since the two objects are of the same cluster,
%the new value should still be large.
%In comparison, 
%both the similarity between $\bmx_1$ and $\bmx_2$ and the one between $\bmx_2$ and $\bmx_3$
%should be rectified, as these distance-based similarities are ineffective.

%In the multi-scale data,
%different clusters may have different sizes, densities or even geometric structures.
The similarity between two objects describes the degree to which they share common characteristics.
The more similar they are, 
the more likely that one object can be represented by the other. 
Therefore,
to depict the relationships between objects in multi-scale data,
each object is linearly characterized by other objects,
assuming the well-known linear subspace model~\cite{liu2013robust}.

We generate $p$ {\pev}s using PI. 
%just as a non-linear manifold can be locally approximated by linear subspaces.
%First, these vectors, which retain the effects of dominant eigenvectors,
%can certainly retain the original accurate similarities between objects.
%Second, they absorb the cluster-separation information from the seemingly ``less important'' eigenvectors,
%which further provides a reliable source of information to rectify the erroneous similarities.
Let $X\in \mathcal{R}^{p\times n}$ be a matrix whose rows are the {\pev}s.
The $q$-th column of $X$ can be taken as a feature vector $\bmx_q$ of an object $x_q$.
We normalize the column vectors of $X$ such that $\bmx_q^T \bmx_q = 1 \; \forall 1 \leq q \leq n$.
We determine a coefficient matrix $Z \in \mathcal{R}^{n \times n}$ by
\begin{equation}
\label{eq:nonoise}
X = XZ,\;\;\; \text{s.t. } diag(Z) = 0.
\end{equation} 
One can interpret $Z_{ij}$ 
as a value that reflects how well object $x_i$ characterizes object $x_j$.
The constraint $diag(Z) = 0$ avoids the trivial solution of $Z$ equals the identity matrix.
For simplicity, we do not explicitly mention this constraint in the rest of the paper.

As indicated by previous works~\cite{ye2016fuse}, the generated pseudo-eigenvectors are likely to be noise-corrupted.
We thus extend Equation~\ref{eq:nonoise} by introducing a noise matrix $O$, giving:
%However, although the pseudo-eigenvectors inherit useful cluster-separation information,
%they may also be contaminated by noise.
%Thus a matrix $O$ is introduced to capture the noise,
\begin{equation}
X = XZ + O.
\label{eq:O}
\end{equation} 
%The TKNN graph conveys information on whether two objects belong to the same cluster or not,

As we have explained, the TKNN graph  conveys useful clustering information, bringing highly
correlated objects that are located at distant far ends of a cluster together.
We thus use the TKNN graph to regularize matrix $Z$.
We derive the following objective function:
%Since our objective is to derive a $Z$ which can better reflect the true similarities between objects,
\comment{
\begin{equation}
%\label{eq:obj}
\min_Z ||O||_F^2+\lambda_1||Z||_F^2 + \lambda_2||Z-\mathcal{W}_K||_F^2,
s.t., X = XZ+O,
\end{equation}
}
%By substituting $O$, we derive
\begin{equation}
\label{eq:obj_constraint}
\min_Z ||X-XZ||_F^2 + \alpha_1 ||Z||_F^2 + \alpha_2 ||Z-\mathcal{W}||_F^2,
\end{equation}
where $\alpha_1 > 0,\alpha_2 \geq 0$ are two 
weighting factors that adjust the relative weights of the three components that constitute
the objective function.
The objective function consists of three terms.
The first term aims to reduce the noise matrix $O$ (see Equation~\ref{eq:O}),
the second term is the Frobenius norm on $Z$, and
%that restricts any item in $Z$ from being dominant.
the third term regularizes $Z$ by the TKNN graph.
%For simplicity, as in~\cite{lu2012robust},
%we remove the constraint and formulate the problem as
%\begin{equation}
%\label{eq:obj}
%\min_Z ||X-XZ||_F^2 + \lambda_1 ||Z||_F^2 + \lambda_2 ||Z-\mathcal{W}_K||_F^2.
%\end{equation}
%$\lambda_1$ and $\lambda_2$ are two parameters to balance the effects of three parts.
A closed-form solution, $Z^*$, to the optimization problem is
\begin{equation}
\label{eq:solution}
Z^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^TX+\alpha_2\mathcal{W}).
\end{equation}

\subsection*{Grouping Effect}
For an object $x_p$, 
let $\bmz_p$ be the $p$-th column of the coefficient matrix $Z$.
We interpret the entries of $\bmz_p$ as the coefficients that express $x_p$ as a linear combinations
of other objects. 
Previous works~\cite{lu2012robust,lu2013correlation,hu2014smooth} have shown that if $Z$ has {\it grouping effect}, then performing spectral 
clustering based on $Z$ would be effective. 
Intuitively, $Z$ has grouping effect if, given two {\it highly correlated} objects $x_i$ and $x_j$,
their characterization of other objects are similar.
Existing works mostly consider {\it high correlation} between objects as {\it high similarity} of their
feature vectors. With ROSC, we consider object similarity in terms of both feature similarity and 
reachability similarity. 
Feature similarity is measured by the objects' feature vectors as given by the columns of matrix $X$.
Reachability similarity is measured by the columns of matrix $\mathcal{W}$, 
each of which shows the reachability of an object to all others. 
Formally,



%It has been shown that the first two terms in the objective function decide the \emph{grouping effect} of $Z$~\cite{lu2012robust}.
%In Problem~\ref{eq:obj}, the first two terms decides whether $Z$ has the grouping effect~\cite{lu2012robust} defined as follows.
%i.e., the more highly correlated two objects are,
%the larger weight one will have in characterizing the other~\cite{lu2012robust}.

\begin{definition}
\label{def:grouping}
\textbf{(Grouping effect)}. 
Given a set of objects $\mathcal{X} = \{x_1, x_2,..., x_n\}$,
let $\bmw_q$ be the $q$-th column of $\mathcal{W}$. 
Further, let $\xarrow{i}{j}$ denote the condition:
(1) $\bmx_i^T \bmx_j \rightarrow 1$ and 
(2) $\lVert \bmw_i - \bmw_j \rVert_2 \rightarrow 0$.
A Matrix $Z$ is said to have grouping effect
if
\[
\xarrow{i}{j} \Rightarrow |Z_{ip} - Z_{jp}| \rightarrow 0\; \forall 1 \leq p \leq n.
\]
%for an arbitrary object $\bmx$ and its associated coefficient vector $\bm{z}$,
%If $\bmx_i\rightarrow \bmx_j$,
%then $z_{pi}\rightarrow z_{pj}$,
%where $z_{pi}$ and $z_{pj}$ are the $i$th and $j$th entry in $\bm{z}_p$ respectively.
%Then we say the self-representation matrix $Z$
%has the grouping effect.
%\hfill$\Box$
\end{definition}

Our next task is to prove that the optimal solution $Z^*$ (as given in Equation~\ref{eq:solution})
% of Equation~\ref{eq:obj_constraint}
has the grouping effect.
In the following discussion, we use $\bmz_q^*$ to denote the $q$-th column vector of $Z^*$.

\begin{lemma}
\label{lemma1}
Given a set of objects $\mathcal{X}$,
the matrix
$X\in \mathcal{R}^{p\times n}$ that is composed of the {\pev}s as rows,
 the reachability matrix $\mathcal{W}$,
 and the optimal soution $Z^*$ of Equation~\ref{eq:obj_constraint},
\begin{equation}
\label{eq:zi}
Z_{ip}^* = \frac{\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*) + \alpha_2 \mathcal{W}_{ip}}{\alpha_1+\alpha_2}, \;\;\; \forall 1 \leq i, p \leq n.
\end{equation}
\end{lemma}

\begin{proof}
For $1 \leq p \leq n$,
let $J(\bm{z}_p) =  ||\bm{x}_p-X\bm{z}_p||_2^2 + \alpha_1 ||\bm{z}_p||_2^2 + \alpha_2 ||\bm{z}_p-\bm{w}_p||_2^2$.
Since $Z^*$ is the optimal solution of Equation~\ref{eq:obj_constraint}, we have $\frac{\partial{J}}{\partial{Z}_{ip}}|_{\bm{z}_p = \bm{z}_p^*} = 0\; \forall 1\leq i \leq n$.
Hence, $-2\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*)+2\alpha_1Z_{ip}^*+2\alpha_2(Z_{ip}^*-\mathcal{W}_{ip}) = 0$,
which induces Equation~\ref{eq:zi}.
\end{proof}

%\begin{lemma}
%\label{lemma1}
%Given a set of objects $X\in \mathcal{R}^{d\times n}$ and a TKNN graph $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathcal{W}_K)$,
%let $\bm{x}_p$ be an arbitrary object and $\bm{w}_p$ be the column vector in $\mathcal{W}_K$ describing the connectivity of $\bmx_p$.
%Each item $z_{pi}^*$ in the optimal solution $\bm{z}_p^*$ to the problem 
%$\min_{\bm{z}} ||\bm{x}_p-X\bm{z}_p||_2^2 + \lambda_1 ||\bm{z}_p||_2^2 + \lambda_2 ||\bm{z}_p-\bm{w}_p||_2^2$ is
%\begin{equation}
%\label{eq:zi}
%z_{pi}^* = \frac{\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*) + \lambda_2 w_{pi}}{\lambda_1+\lambda_2},
%\end{equation}
%where $w_{pi} = 1$, if $\bm{x_p}$ and $\bm{x}_i$ are reachable; $0$, otherwise. 
%
%Proof. Let $J(\bm{z}_p) =  ||\bm{x}_p-X\bm{z}_p||_2^2 + \lambda_1 ||\bm{z}_p||_2^2 + \lambda_2 ||\bm{z}_p-\bm{w}_p||_2^2$.
%Since $\bm{z}_p^*$ is the optimal solution, then $\frac{\partial{J}}{\partial{z}_{pi}}|_{\bm{z}_p = \bm{z}_p^*} = 0$.
%Thus we have $-2\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*)+2\lambda_1z_{pi}^*+2\lambda_2(z_{pi}^*-w_{pi}) = 0$,
%which induces Eq.~\ref{eq:zi}.
%\end{lemma}

\comment{
Eq.~\ref{eq:zi} calculates the weight of object $\bm{x}_i$ in characterizing $\bm{x}$.
For $w_i$, if $\bm{x}$ and $\bm{x}_i$ are reachable in the TKNN graph, $w_i = 1$; otherwise, $w_i = 0$. 
Eq.~\ref{eq:zi} rectifies the ineffective similarity as follows.
When $\bm{x}$ and $\bm{x_i}$ are far away from each other in the feature space
but reachable in the TKNN graph,
$z_i$ will be increased by $w_i = 1$.
%which rectifies the original incorrect similarity value between them.
Moreover, if $\bm{x}$ and $\bm{x}_i$ are highly correlated,
the first two terms in the problem can decide a large $z_i$,
even in the case that they are unreachable.
%$z_i$ can still keep large with a small $\lambda_2$.
In summary, Eq.~\ref{eq:zi} can not only hold the original accurate similarities but also rectify the incorrect ones.

\noindent{\small$\bullet$}
For any two objects dissimilar in the feature space but connected in the TKNN graph, 
their similarity will be increased.

\noindent{\small$\bullet$}
For any two objects dissimilar in the feature space and disconnected in the TKNN graph, 
their similarity will be further decreased.

\noindent{\small$\bullet$}
For any two objects similar in the feature space and connected in the TKNN graph,
their similarity will be further increased.

\noindent{\small$\bullet$}
For any two objects similar in the feature space but disconnected in the TKNN graph,
their similarity will be decreased. In this case,
provided that the raw similarity is effective already,
even though the new value will be decreased,
but it will be still
}

\begin{lemma}
\label{lemma2}
%Given a set of objects $X\in R^{d\times n}$ and a TKNN graph $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathcal{W}_K)$,
%let $\bm{x}_p$ be an arbitrary object, 
%$\bm{w}_p$ be the column vector in $\mathcal{W}_K$ describing the connectivity of $\bm{x}_p$, and
%$\bm{z}_p^*$ be the optimal solution to the problem 
%$\min_{\bm{z}_p} ||\bm{x}_p-X\bm{z}_p||_2^2 + \lambda_1 ||\bm{z}_p||_2^2 + \lambda_2 ||\bm{z}_p-\bm{w}_p||_2^2$.
%Assume all the objects have been normalized.
%For any two objects $\bm{x}_i$ and $\bm{x}_j$,
$\forall 1 \leq i, j, p \leq n$,
\begin{equation}
\label{eq:norm}
|Z_{ip}^*-Z_{jp}^*| \leq \frac{c\sqrt{2(1-r)} + \alpha_2|\mathcal{W}_{ip}-\mathcal{W}_{jp}|}{\alpha_1+\alpha_2},
\end{equation}
where $c = \sqrt{1+\alpha_2||\bm{w}_p||_2^2}$ and $r = \bm{x}_i^T\bm{x}_j$.
\end{lemma}

\begin{proof}
From Equation~\ref{eq:zi}, we have 
\begin{equation}
\nonumber
Z_{ip}^*-Z_{jp}^* = \frac{(\bm{x}_i^T - \bm{x}_j^T)(\bm{x}_p-X\bm{z}_p^*) + \alpha_2 (\mathcal{W}_{ip}-\mathcal{W}_{jp})}{\alpha_1+\alpha_2}.
\end{equation}
That implies 
\begin{small}
\begin{equation}
\label{eq:zizj}
\begin{split}
|Z_{ip}^*-Z_{jp}^*| & \leq \frac{|(\bm{x}_i^T - \bm{x}_j^T)(\bm{x}_p-X\bm{z}_p^*)| + \alpha_2 |(\mathcal{W}_{ip}-\mathcal{W}_{jp})|}{\alpha_1+\alpha_2}\\
& \leq \frac{||(\bm{x}_i^T - \bm{x}_j^T)||_2||(\bm{x}_p-X\bm{z}_p^*)||_2 + \alpha_2 |(\mathcal{W}_{ip}-\mathcal{W}_{jp})|}{\alpha_1+\alpha_2}\\
\end{split}
\end{equation}
\end{small}

Since the column vectors of $X$ are normalized (i.e., $\bmx_q^T \bmx_q = 1 \; \forall 1 \leq q \leq n$) , we have
$||(\bm{x}_i^T - \bm{x}_j^T)||_2 = \sqrt{2(1-r)}$,
where $r = \bm{x}_i^T\bm{x}_j$.
%measuring the closeness between $\bm{x}_i$ and $\bm{x}_j$ in the feature space.
%As $\bm{z}_p^*$ is the optimal solution, 
As $Z^*$ is the optimal solution of Equation~\ref{eq:obj_constraint}, we have
\begin{equation}
\begin{split}
J(\bm{z}_p^*) & = ||\bm{x}_p-X\bm{z}_p^*||_2^2 + \alpha_1 ||\bm{z}_p^*||_2^2 + \alpha_2 ||\bm{z}_p^*-\bm{w}_p||_2^2 \leq  \\
J(\bm{0}) & = ||\bm{x}_p||_2^2 + \alpha_2 ||\bm{w}_p||_2^2 = 1 + \alpha_2 ||\bm{w}_p||_2^2.
\end{split}
\end{equation}
Hence, $||\bm{x}_p-X\bm{z}_p^*||_2 \leq \sqrt{1 + \alpha_2 ||\bm{w}_p||_2^2} = c$.
Equation~\ref{eq:zizj} can be further simplified as
\begin{equation}
\nonumber
|Z_{ip}^*-Z_{jp}^*| \leq \frac{c\sqrt{2(1-r)}+ \alpha_2 |(\mathcal{W}_{ip}-\mathcal{W}_{jp})|}{\alpha_1+\alpha_2}.
\end{equation}
\end{proof}

\begin{lemma}
Matrix $Z^*$ has grouping effect.
\label{lemma:z-star}
\end{lemma}
\begin{proof}
Given two objects $x_i$ and $x_j$ such that $\xarrow{i}{j}$,
we have,  %by definition, 
(1) $\bmx_i^T \bmx_j \rightarrow 1$ and (2) $||\bmw_{i}-\bmw_{j}||_2 \rightarrow 0$.
These imply
$r = \bmx_i^T \bmx_j \rightarrow 1$ and  $|\mathcal{W}_{ip}-\mathcal{W}_{jp}| \rightarrow 0$.
Hence, the two terms of the numerator of the R.H.S of Equation~\ref{eq:norm} are close to 0. 
Therefore, $|Z_{ip}^*-Z_{jp}^*| \rightarrow 0$ and thus $Z^*$ has grouping effect.
\end{proof}

Indeed, Equation~\ref{eq:norm} shows how our algorithm ROSC enhances the effectiveness of 
spectral clustering on multi-scale data. 
Comparing with traditional approaches, which focus on feature similarity, ROSC uses $Z^*$
to integrate feature similarity  ($r$) with
reachability similarity ($|\mathcal{W}_{ip}-\mathcal{W}_{jp}|$).
In particular, two distant objects $x_i$ and $x_j$ of a cluster may not share a strong feature similarity.
This leads to a small $r$ and traditional approaches will likely put them into separate clusters.
On the contrary, ROSC considers the strong reachability of the objects
to derive a small value of $|\mathcal{W}_{ip}-\mathcal{W}_{jp}|$, and thus keeping them in the same cluster.
Moreover, for $x_i$ and $x_j$ that belong to two different dense clusters but happen to be close in 
space (i.e., $x_i$ and $x_j$ have strong feature similarity), 
traditional approaches may inadvertently merge them into the same cluster. 
ROSC, however, would discover their low reachability (via the mutual-KNN relation)
and derive a large value of $|\mathcal{W}_{ip}-\mathcal{W}_{jp}|$.
This regulates matrix $Z^*$ and avoids the incorrect merging.
As we will see in the next section, ROSC's approach 
greatly improves clustering quality and is more robust than other algorithms in handling
multi-scale data.
 
%Lemma~\ref{lemma1} and~\ref{lemma2} prove the grouping effect of $Z^*$ derived by Eq.~\ref{eq:solution}.
%%the weight difference of two objects in characterizing an arbitrary object $\bm{x}$ is bounded.
%Given two objects $\bmx_i$ and $\bmx_j$, if $\bmx_i \rightarrow \bmx_j$, 
%i.e., $\bmx_i^T \bmx_j \rightarrow 1$ and $||w_{pi}-w_{pj}||_2 \rightarrow 0$,
%then $||z_{pi}^*-z_{pj}^*||_2 \rightarrow 0$.
%%which shows the grouping effect of $Z$ derived by Eq.~\ref{eq:solution}.
%%However, in the case of (1) $\bm{x}_i^T\bm{x}_j = 0$ but $w_i=w_j=1$ and 
%%(2) $\bm{x}_i^T\bm{x}_j = 1$ but $||w_i-w_j||_2=1$,
%%$||z_i^*-z_j^*||_2$ can still be small with an appropriate setting on $\lambda_1$ and $\lambda_2$.
%%Further, since $Z$ can not only retain the accurate similarities but also rectify the incorrect ones, 
%%In other words, objects in the same cluster will be better reflected in the rectified matrix.
%%Such grouping effect together with The rectification ability could guarantee a more robust clustering performance.
%We then summarize how the TKNN graph rectifies the raw similarity matrix.
%Given any two objects $\bmx_i$ and $\bmx_j$,
%\begin{enumerate}[label=(\arabic*), leftmargin=*]
%\setlength{\itemsep}{0pt}
%\setlength{\parsep}{0pt}
%\setlength{\parskip}{0pt}
%\item $\bmx_i^T \bmx_j \rightarrow 0$, $\bmx_i$ and $\bmx_j$ are reachable, the effect of $S_{ij}$ will be increased.
%\item $\bmx_i^T \bmx_j \rightarrow 0$, $\bmx_i$ and $\bmx_j$ are unreachable, the effect of $S_{ij}$ will be further decreased.
%\item $\bmx_i^T \bmx_j \rightarrow 1$, $\bmx_i$ and $\bmx_j$ are reachable, the effect of $S_{ij}$ will be further increased.
%\item $\bmx_i^T \bmx_j \rightarrow 1$, $\bmx_i$ and $\bmx_j$ are unreachable, the effect of $S_{ij}$ will be decreased.
%\end{enumerate}
%Among the four cases,
%$Z$ reserves the efficacy of effective similarities by (2) and (3)
%while it enhances the efficacy of ineffective similarities by (1) and (4). 
%Thus spectral clustering based on $Z$ will be more robust.

\comment{
\noindent{\small$\bullet$}
$\bmx_i^T \bmx_j \rightarrow 0$ but reachable, $S_{ij}$ will be increased.

\noindent{\small$\bullet$}
%For any two objects dissimilar in the feature space and disconnected in the TKNN graph, their similarity will be further decreased.
$\bmx_i^T \bmx_j \rightarrow 0$ and unreachable, $S_{ij}$ will be further decreased.

\noindent{\small$\bullet$}
%For any two objects similar in the feature space and connected in the TKNN graph, their similarity will be further increased.
$\bmx_i^T \bmx_j \rightarrow 1$ and reachable, $S_{ij}$ will be further increased.

\noindent{\small$\bullet$}
$\bmx_i^T \bmx_j \rightarrow 1$ but unreachable, $S_{ij}$ will be decreased.
}

\subsection*{ROSC: Robust Spectral Clustering}
%The coefficient matrix $Z$ take advantage of both cluster-separation information in all the eigenvectors
%and the TkNN graph, which not only retains the original accurate similarities but also rectifies the incorrect ones.

We note that the matrix $Z^*$ obtained may be asymmetric and it may contain negative values.
To construct a matrix of object similarity, a common fix~\cite{liu2013robust,lu2012robust} is to 
compute $\tilde{Z} = (|Z^*|+|(Z^*)^T|)/2$.
After $\tilde{Z}$ is computed, ROSC executes a standard spectral clustering method
(e.g., NCuts) using $\tilde{Z}$ as the similarity matrix in place of $S$.
It can be proved that $|Z^*|$, $|(Z^*)^T|$, and hence $\tilde{Z}$ all have grouping effect.
%Due to space limitations, readers are referred to [XXX] for the proofs. 
Finally, ROSC is summarized in Algorithm~\ref{alg}.


\begin{lemma}
Matrix $|Z^*|$ has grouping effect.
\label{lemma:z-star-abs}
\end{lemma}
\begin{proof}
Given two objects $x_i$ and $x_j$,
we have 
$\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| \leq |Z_{ip}^*-Z_{jp}^*|$.
From Lemma~\ref{lemma:z-star},
$Z^*$ has grouping effect, i.e.,
if $x_i \rightarrow x_j$, $|Z_{ip}^*-Z_{jp}^*| \rightarrow 0$.
Thus $\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| \rightarrow 0$ and 
$|Z^*|$ has grouping effect.
\end{proof}

\begin{lemma}
\label{lemma3}
$(Z^*)^T$ and $|(Z^*)^T|$ have grouping effect. 
\begin{proof}
The problem is equivalent to if $x_i \rightarrow x_j$, $Z^*_{pi} \rightarrow Z^*_{pj}$.
From Lemma~\ref{lemma1},
\begin{equation}
\nonumber
z_{pi}^*-z_{pj}^* = \frac{\bm{x}_p^T ( \bmx_i - \bmx_j - X(\bm{z}_i^*-\bm{z}_j^*)) + \alpha_2 (W_{pi}-W_{pj})}{\alpha_1+\alpha_2}.
\end{equation}
Since $\bm{z}_i^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_i+\alpha_2\bm{w}_i),\bm{z}_j^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_j+\alpha_2\bm{w}_j)$,
let $Y = X(X^TX + \alpha_1I + \alpha_2I)^{-1}$. Then
\begin{equation}
\begin{split}
|Z_{pi}^*-Z_{pj}^*| & \leq \frac{||\bmx_p^T(\bm{x}_i - \bm{x}_j)||_2 + ||\bmx_p^TX(\bm{z}_i^*-\bm{z}_j^*)||_2 + \alpha_2 |(W_{pi}-W_{pj})|}{\alpha_1+\alpha_2}\\
& \leq \frac{||\bmx_p^T(\bm{x}_i - \bm{x}_j)||_2 + ||\bmx_p^TYX^T(\bmx_i-\bmx_j)||_2}{\alpha_1+\alpha_2}\\
& + \frac{\alpha_2||\bmx_p^TY(\bm{w}_i - \bm{w}_j)||_2 + \alpha_2 |W_{pi}-W_{pj}|}{\alpha_1+\alpha_2}\\
\end{split}
\end{equation}
If $x_i \rightarrow x_j$, i.e., $\bmx_i^T\bmx_j \rightarrow 1$ and $||\bm{w}_i - \bm{w}_j||_2 \rightarrow 0$, 
we have
$||\bm{x}_i - \bm{x}_j||_2 \rightarrow 0$ and $|W_{pi}-W_{pj}| \rightarrow 0$.
Then $|Z_{pi}^*-Z_{pj}^*| \rightarrow 0$ and
$(Z^*)^T$ has grouping effect.
Since $\bigl||Z_{pi}^*|-|Z_{pj}^*|\bigr| \leq |Z_{pi}^*-Z_{pj}^*|$, $|(Z^*)^T|$ also has grouping effect.
\end{proof}
\end{lemma}

\begin{lemma}
\label{lemma4}
Matrix $\tilde{Z}$ has grouping effect. 
\begin{proof}
From Lemma~\ref{lemma:z-star-abs} and~\ref{lemma3},
both $\lvert Z^*\rvert$ and $\lvert (Z^*)^T\rvert$ have the grouping effect.
Since $\tilde{Z} = (|Z^*|+|(Z^*)^T|)/2$,
\begin{equation}
\begin{split}
\lvert \tilde{Z}_{ip} - \tilde{Z}_{jp}\rvert & = \frac{\bigl| (|Z^*_{ip}|+|Z^*_{pi}|) - (|Z^*_{jp}|+|Z^*_{pj}|)\bigr|}{2} \\
& \leq \frac{\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| + \bigl||Z_{pi}^*|-|Z_{pj}^*|\bigr|}{2}
\end{split}
\end{equation}
If $x_i \rightarrow x_j$,
both $\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| \rightarrow 0$ and $\bigl||Z_{pi}^*|-|Z_{pj}^*|\bigr| \rightarrow 0$,
so $\lvert \tilde{Z}_{ip} - \tilde{Z}_{jp}\rvert \rightarrow 0$ and
$\tilde{Z}$ has grouping effect.
\end{proof}
\end{lemma}


\comment{
\begin{lemma}
\label{lemma3}
$(Z^*)^T$ has the grouping effect. 

Proof. The problem is equivalent to if $x_i \rightarrow x_j$, $Z^*_{pi} \rightarrow Z^*_{pj}$.
From Lemma~\ref{lemma1},
\begin{equation}
\nonumber
z_{pi}^*-z_{pj}^* = \frac{\bm{x}_p^T ( \bmx_i - \bmx_j - X(\bm{z}_i^*-\bm{z}_j^*)) + \alpha_2 (W_{pi}-W_{pj})}{\alpha_1+\alpha_2}.
\end{equation}
Since $\bm{z}_i^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_i+\alpha_2\bm{w}_i),\bm{z}_j^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_j+\alpha_2\bm{w}_j)$,
let $Y = X(X^TX + \alpha_1I + \alpha_2I)^{-1}$. Then
\begin{equation}
\begin{split}
||Z_{pi}^*-Z_{pj}^*||_2 & \leq \frac{||\bmx_p^T(\bm{x}_i - \bm{x}_j)||_2 + ||\bmx_p^TX(\bm{z}_i^*-\bm{z}_j^*)||_2 + \alpha_2 ||(W_{pi}-W_{pj})||_2}{\alpha_1+\alpha_2}\\
& \leq \frac{||\bmx_p^T(\bm{x}_i - \bm{x}_j)||_2 + ||\bmx_p^TYX^T(\bmx_i-\bmx_j)||_2}{\alpha_1+\alpha_2}\\
& + \frac{\alpha_2||\bmx_p^TY(\bm{w}_i - \bm{w}_j)||_2 + \alpha_2 ||W_{pi}-W_{pj}||_2}{\alpha_1+\alpha_2}\\
\end{split}
\end{equation}
If $x_i \rightarrow x_j$, i.e., $\bmx_i^T\bmx_j \rightarrow 1$ and $||\bm{w}_i - \bm{w}_j||_2 \rightarrow 0$, 
we have
$||\bm{x}_i - \bm{x}_j||_2 \rightarrow 0$ and $||W_{pi}-W_{pj}||_2 \rightarrow 0$.
Then $||Z_{pi}^*-Z_{pj}^*||_2 \rightarrow 0$,
which proves the grouping effect of $(Z^*)^T$.
%\begin{equation}
%\begin{split}
%||\bmx_p^TX(\bm{z}_i^*-\bm{z}_j^*)||_2 & \leq ||\bmx_p^TY(X^T(\bmx_i-\bmx_j) +\alpha_2(\bm{w}_i - \bm{w}_j))||_2\\
%& \leq ||\bmx_p^TYX^T(\bmx_i-\bmx_j)||_2 +\alpha_2||\bmx_p^TY(\bm{w}_i - \bm{w}_j)||_2\\
%\end{split}
%\end{equation}
\end{lemma}

\begin{lemma}
\label{lemma4}
$\tilde{Z}$ has the grouping effect. 

Proof. From Lemma~\ref{lemma2} and~\ref{lemma3},
both $Z^*$ and $(Z^*)^T$ have the grouping effect,
which can be easily extended to
$|Z^*|$ and $|(Z^*)^T|$.
Since $\tilde{Z} = (|Z^*|+|(Z^*)^T|)/2$,
$\tilde{Z}$ also has the grouping effect.
\end{lemma}

To this end, we summarize ROSC as follows.
ROSC first computes the TKNN graph $\mathcal{G}$
and the associated weight matrix $\mathcal{W}_K$. Then it applies power iteration to generate $p$
pseudo-eigenvectors that form a $p \times n$ matrix $X$.
After whitening and normalization on $X$,
the coefficient matrix $Z^*$ can be calculated by solving Eq.~\ref{eq:solution},
which further leads to the construction of a rectified similarity matrix $\tilde{Z}$.
Since $\tilde{Z}$ has the grouping effect, 
the standard spectral clustering methods (e.g., NCuts) will be finally applied to derive more robust clustering results.
The time complexity of ROSC will be no more than the standard spectral clustering methods,
which is $O(n^3)$ in general.
In the future, we will attempt to improve it. 
}

\begin{algorithm}
\begin{small}
\caption{ROSC}
\label{alg}
\begin{algorithmic}[1]
\Require $S$, $k$.
\Ensure $\mathcal{C} = \{C_1, ..., C_k\}$
\State Compute TKNN graph $\mathcal{G}$ and reachability matrix $\mathcal{W}$
\State Normalize the similarity matrix $S$ by $W = D^{-1}S$
%\For $j \leftarrow 1$ do
%\State$t = 0$
%\Repeat
%\State $v_j^{t+1} \leftarrow \frac{Wv_j^t}{||Wv_j^t||_1}$
%\State $ \delta^{t+1} \leftarrow |v_j^{t+1} - v_j^t|$
%\State $t$++
%\Until $||\delta_j^t+1 - \delta_j^t||_{max} \leq \epsilon$ or $t\geq T$
%\EndFor
\State Apply PI on $W$ and generate $p$ pseudo-eigenvectors $\{\bm{v}_r\}_{r=1}^p$
\State $X = \{\bm{v}_1^T; \bm{v}_2^T; ...; \bm{v}_p^T\}$; $X$ = whiten($X$)
\State Normalize each object feature vector
\State Solve Eq.~\ref{eq:solution} to obtain the coefficient matrix $Z^*$
\State Construct a rectified similarity matrix $\tilde{Z} = (|Z^*| + |Z^*|^T)/2$
\State Run standard spectral clustering methods, e.g., NCuts, with $\tilde{Z}$ as the
similarity matrix to obtain a clustering $\mathcal{C} = \{C_r\}_{r=1}^k$
%\State Decode $\{C_r\}_{r=1}^k$ from $\{{\bm z_r}\}_{r=1}^k$
\State \Return $\mathcal{C} = \{C_1, ..., C_k\}$
\end{algorithmic}
\end{small}
\end{algorithm}









==> tex/algorithm_report1.tex <==
\section{Algorithm}
\label{sec:algorithm}

In this section we describe our ROSC algorithm. Figure~\ref{figure:flow_graph}(c) shows a 
flow diagram of ROSC. ROSC follows the basic pipeline of spectral clustering except that
it generates a coefficient matrix $Z$ 
%(shown in the red box of the diagram) 
and feeds it
 into the clustering pipeline in place of
the similarity matrix $S$. 
The objective is to find a  $Z$ that possesses  grouping effect. 
To achieve that, ROSC uses PI to obtain {\pev}s from which a basic $Z$ is derived.
Next, it generates the TKNN graph with which $Z$ is rectified. 
In the following, we discuss how $Z$ is derived from the {\pev}s, define the TKNN graph,
describe the rectification process, 
and prove that the resulting $Z$ has the desired grouping effect. 

%
%In this section, we propose a \textbf{RO}bust \textbf{S}pectral \textbf{C}lustering method ROSC. 
%Instead of directly performing spectral clustering on the given similarity matrix, 
%it constructs a new matrix that reserves the efficacy of effective similarities 
%and rectifies ineffective ones in the raw similarity matrix.
%The new matrix will lead to a more robust spectral clustering.

\comment{
\subsection{Model overview}
The overall framework of ROSC is summarized as follows.

First, generate a set of pseudo-eigenvectors.
Since the standard spectral clustering methods using only the dominant eigenvectors may fail 
in the data containing multi-scale clusters,
we generate a set of pseudo-eigenvectors to fuse more useful cluster-separation information.

Second, rectify the given similarity matrix.
The failure of spectral clustering on multi-scale data originates from the inaccurate similarity matrix.
Therefore, we rectify the matrix and aim to achieve a new one
that can more accurately reflect the true similarities between objects.
%This is a major problem to be addressed.

Third, perform spectral clustering.
After rectification, the new similarity matrix will be more accurate and it will be safer to perform spectral clustering. 

These three steps will lead to robust clustering results and next we introduce each step in detail.
}

\subsection*{Pseudo-Eigenvectors}
\label{sec:sec:pseudo}
Given a similarity matrix $S$, we normalize it by $D^{-1}S$ and apply PI to obtain {\pev}s.
%When dealing with multi-scale data,
%spectral clustering
%using only the top-$k$ eigenvectors may fail while some other eigenvectors may be useful~\cite{lin2010power}.
%Therefore, it is necessary to fuse the discriminative cluster-separation information in all eigenvectors
%and PI provides such fusion by returning a pseudo-eigenvector.
%However, when the number of clusters is large,
%a single pseudo-eigenvector is insufficient due to the cluster-collision problem. 
%%Since PI returns a pseudo-eigenvector that is a combination of all the eigenvectors,
Similar to~\cite{ye2016fuse},
we run PI multiple times with different random initial vectors to generate a set of {\pev}s, 
which maps each object into a low dimensional embedding.
Note that small {\ev}s are {\it shrunk} by PI~\cite{lin2010power}.
%\footnote{From Equation~\ref{eq:pi}, we see that the $i$-th 
%largest \ev\ is 
%shrunk at a rate of $\lambda_i/\lambda_1$ per iteration.}.
To alleviate the shrinkage of small {\ev}s,
we follow the approach of~\cite{huang2014diverse}
and gradually decrease the number of iterations executed in PI as more {\pev}s are obtained. 

Since the {\pev}s approximate the most dominant {\ev}, they could be similar. 
To reduce this redundancy,
whitening~\cite{kessy2017optimal} is used to make the pseudo-eigenvectors uncorrelated.
Moreover, noise in the {\pev}s are reduced 
by a rectification process, which will be discussed later.

\comment{
First, we generate a set of pseudo-eigenvectors using different random vectors $\bm{v}_0$.
From Eq.~\ref{eq:v0}, $\bm{v}_0$ can be represented by the subspace spanned by all the eigenvectors.
Suppose $\bm{e}_i$ is an informative eigenvector with a relatively small eigenvalue $\lambda_i$.
Given a $\bm{v}_0$, if it has a dominant component in the direction of $\bm{e}_i$, 
i.e., the associated coefficient $c_i$ is large, 
with an appropriate number of iterations, $c_i\lambda_i^t\approx c_2\lambda_2^t$,
the effect of $\bm{e}_i$ will be finally retained in the pseudo-eigenvector.
Therefore, multiple pseudo-eigenvectors generated by different $\bm{v}_0$
may increase the chance to hold all the informative eigenvectors.

Second, we can control the number of iterations in PI.
In PIC, the \emph{velocity} and \emph{acceleration} at the $t$-th iteration are respectively defined as
$\bm{\delta}_t = \bm{v}_t - \bm{v}_{t-1}$ and $\bm{\epsilon}_t = \bm{\delta}_t-\bm{\delta}_{t-1}$.
A threshold $\epsilon$ is introduced to measure the acceleration change in two consecutive iterations 
and stop PI when $|\bm{\epsilon}_t-\bm{\epsilon}_{t-1}|<\epsilon$.
However,
since the effect of eigenvectors corresponding to smaller eigenvalues will shrink as $t$ increases,
we can decrease the number of iterations by gradually increasing the $\epsilon$ value,
which provides another way to keep useful information in ``less important'' eigenvectors. 
}

\subsection*{Transitive {\it K} Nearest Neighbor (TKNN) Graph}

%\begin{figure}
%    \centering
%        \includegraphics[width = 0.8\linewidth]{figure/example1.eps}
%        \caption{An toy example}
%        \label{figure:example1}
%\end{figure}

%The \emph{$K$ nearest neighbor} (KNN) graph is generally used to depict the most adjacent relations between objects,
%in which the linked objects are generally assumed to share common characteristics.
%Given a set of objects $\mathcal{X} = \{\bm{x}_1,\bm{x}_2,...,\bm{x}_n\}$,
%the KNN graph $G_{K} = (V, E)$ is a graph with $V = \mathcal{X}$ and $E = \{e_{ij}\}$.
%%An edge $e_{ij}$ between $\bm{x}_i$ and $\bm{x}_j$ indicates
%%$x_j \in N_K(\bm{x}_i)$ or $x_i \in N_K(\bm{x}_j)$,
%%where $N_K(\bm{x}_i)$ denotes the set of $K$ nearest neighbors of $\bm{x}_i$.
%%at least one of the two end nodes is in the $K$ nearest neighborhood of the other.
%%However, the $K$ nearest neighborhood relation is not symmetric,
%%i.e., $x_j \in N_K(\bm{x}_i)$ is inequivalent to $x_i \in N_K(\bm{x}_j)$, 
%Some previous work~\cite{yin2016laplacian} simply considers $e_{ij}$
%exists when $\bmx_j \in N_K(\bmx_i)$ or $x_i \in N_K(\bmx_j)$,
%where $N_K(\bmx_i)$ denotes the set of $K$ nearest neighbors of $\bmx_i$.
%However,
%in the case of data containing multi-scale clusters,
%such definition may lead to an edge between
%two objects in different clusters.
%Fig.~\ref{figure:example1} shows an toy example which consists of two multi-scale clusters
%marked by ``$\times$" and ``$+$" respectively.
%For object $\bmx_1$,
%object $\bmx_2$ is its nearest neighbor.
%But for $\bmx_2$, $\bmx_1$ is far away from it.
%In this case, there will be an edge between $\bmx_1$ and $\bmx_2$ in the traditional KNN graph.
%However, since $\bmx_1$ and $\bmx_2$ belong to different clusters,
%they should not be connected.

Our objective is to capture the high correlations between objects that belong to the same cluster even 
 though the objects could be located at distant far ends of a cluster. 
 These correlations are expressed via a TKNN graph, which is used to 
 regularize the coefficient matrix $Z$.

\begin{definition}
\label{def:nei_relation}
\textbf{(Mutual  $K$-nearest neighbors)}
Let $N_K(x)$ be the set of $K$ nearest neighbors of an object $x$.
Two objects $x_i$ and $x_j$ are said to be mutual $K$-nearest neighbors of each other,
denoted by $x_i \sim x_j$, 
iff $x_i \in N_K(x_j)$ and $x_j \in N_K(x_i)$.
\hfill$\Box$
\end{definition}

%In the case of multi-scale data,
%the KNN graph is sometimes insufficient to reflect whether two objects belong to the same cluster or not.
%For example, objects $\bmx_2$ and $\bmx_3$ in Fig.~\ref{figure:example1} belong to the same cluster, 
%but they are both far away from each other.
%%objects $x_1$ and $x_2$ are in different clusters despite their closeness.
%To construct an effective KNN graph, $\bmx_2$ and $\bmx_3$
%are expected to be linked.
%Therefore,
%the reachability between two objects is introduced.

\begin{definition}
\label{def:reachability}
\textbf{(Reachability)}
Two objects $x_i$ and $x_j$ are said to be reachable from each other
if there exists a sequence of $h \geq 2$ objects 
 $\{x_i = x_{a_1}, \ldots, x_{a_h} = x_j\}$ such that
 $x_{a_r} \sim x_{a_{r+1}}$ for $1 \leq r < h$.
 \hfill$\Box$
\end{definition}

\begin{definition}
\label{def:trans_relation}
\textbf{(Transitive $K$-nearest neighbor (TKNN) graph)}
Given a set of objects $\mathcal{X} = \{x_1, x_2,..., x_n\}$,
the TKNN graph $\mathcal{G}_K = (\mathcal{X},\mathcal{E})$
is an undirected graph
where $\mathcal{X}$ is the set of vertices and $\mathcal{E}$ is the set of edges.
Specifically, the edge ($x_i$, $x_j$) $\in \mathcal{E}$
iff $x_i$ and $x_j$ are reachable from each other.
We represent the TKNN graph by an $n \times n$ {\it reachability matrix}
$\mathcal{W}$ 
whose ($i$,$j$)-entry $\mathcal{W}_{ij} = 1$ if ($x_i$, $x_j$) $\in \mathcal{E}$; 0 otherwise.
\hfill$\Box$
\end{definition}

%We note that mutual-KNN is a symmetric relation and so is reachability. 

%Compared with the traditional KNN graph, 
%the TKNN graph can more accurately reflect 
%whether two objects belong to the same cluster or not.
%It will be used in the next section to rectify the matrix of similarity between objects.
 
\subsection*{Coefficient Matrix}
%In the case of multi-scale data,
%the distance-based similarity is likely to be ineffective. 
%To improve the clustering performance,
%it is necessary to rectify the matrix.
%The rectification should follow two principles.
%First, for the effective similarities, the efficacy should be reserved.
%Second, for the ineffective ones, the efficacy should be enhanced.
%For example,
%the closeness between objects $\bmx_3$ and $\bmx_4$ in Fig.~\ref{figure:example1}
%leads to a large similarity value.
%Since the two objects are of the same cluster,
%the new value should still be large.
%In comparison, 
%both the similarity between $\bmx_1$ and $\bmx_2$ and the one between $\bmx_2$ and $\bmx_3$
%should be rectified, as these distance-based similarities are ineffective.

%In the multi-scale data,
%different clusters may have different sizes, densities or even geometric structures.
The similarity between two objects describes the degree to which they share common characteristics.
The more similar they are, 
the more likely that one object can be represented by the other. 
Therefore,
to depict the relationships between objects in multi-scale data,
each object is linearly characterized by other objects,
assuming the well-known linear subspace model~\cite{liu2013robust}.

We generate $p$ {\pev}s using PI. 
%just as a non-linear manifold can be locally approximated by linear subspaces.
%First, these vectors, which retain the effects of dominant eigenvectors,
%can certainly retain the original accurate similarities between objects.
%Second, they absorb the cluster-separation information from the seemingly ``less important'' eigenvectors,
%which further provides a reliable source of information to rectify the erroneous similarities.
Let $X\in \mathcal{R}^{p\times n}$ be a matrix whose rows are the {\pev}s.
The $q$-th column of $X$ can be taken as a feature vector $\bmx_q$ of an object $x_q$.
We normalize the column vectors of $X$ such that $\bmx_q^T \bmx_q = 1 \; \forall 1 \leq q \leq n$.
We determine a coefficient matrix $Z \in \mathcal{R}^{n \times n}$ by\footnote{We will regularize $Z$ to avoid the trivial solution of $Z$ being the identity matrix.}
\begin{equation}
\label{eq:nonoise}
X = XZ.
\end{equation} 
One can interpret $Z_{ij}$ 
as a value that reflects how well object $x_i$ characterizes object $x_j$.
%To avoid the trivial solution of $Z$ equalling the identity matrix,
%we will regularize $Z$ later.
%For simplicity, we do not explicitly mention this constraint in the rest of the paper.

As indicated by previous works~\cite{ye2016fuse}, the generated pseudo-eigenvectors are likely to be noise-corrupted.
We thus extend Equation~\ref{eq:nonoise} by introducing a noise matrix $O$, giving:
%However, although the pseudo-eigenvectors inherit useful cluster-separation information,
%they may also be contaminated by noise.
%Thus a matrix $O$ is introduced to capture the noise,
\begin{equation}
X = XZ + O.
\label{eq:O}
\end{equation} 
%The TKNN graph conveys information on whether two objects belong to the same cluster or not,

As we have explained, the TKNN graph  conveys useful clustering information, bringing highly
correlated objects that are located at distant far ends of a cluster together.
We thus use the TKNN graph to regularize matrix $Z$.
We derive the following objective function:
%Since our objective is to derive a $Z$ which can better reflect the true similarities between objects,
\comment{
\begin{equation}
%\label{eq:obj}
\min_Z ||O||_F^2+\lambda_1||Z||_F^2 + \lambda_2||Z-\mathcal{W}_K||_F^2,
s.t., X = XZ+O,
\end{equation}
}
%By substituting $O$, we derive
\begin{equation}
\label{eq:obj_constraint}
\min_Z ||X-XZ||_F^2 + \alpha_1 ||Z||_F^2 + \alpha_2 ||Z-\mathcal{W}||_F^2,
\end{equation}
where $\alpha_1 > 0,\alpha_2 \geq 0$ are two 
weighting factors that adjust the relative weights of the three components that constitute
the objective function.
The objective function consists of three terms.
The first term aims to reduce the noise matrix $O$ (see Equation~\ref{eq:O}),
the second term is the Frobenius norm on $Z$, and
%that restricts any item in $Z$ from being dominant.
the third term regularizes $Z$ by the TKNN graph.
%For simplicity, as in~\cite{lu2012robust},
%we remove the constraint and formulate the problem as
%\begin{equation}
%\label{eq:obj}
%\min_Z ||X-XZ||_F^2 + \lambda_1 ||Z||_F^2 + \lambda_2 ||Z-\mathcal{W}_K||_F^2.
%\end{equation}
%$\lambda_1$ and $\lambda_2$ are two parameters to balance the effects of three parts.
A closed-form solution, $Z^*$, to the optimization problem is
\begin{equation}
\label{eq:solution}
Z^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^TX+\alpha_2\mathcal{W}).
\end{equation}

\subsection*{Grouping Effect}
For an object $x_p$, 
let $\bmz_p$ be the $p$-th column of the coefficient matrix $Z$.
We interpret the entries of $\bmz_p$ as the coefficients that express $x_p$ as a linear combinations
of other objects. 
Previous works~\cite{lu2012robust,lu2013correlation,hu2014smooth} have shown that if $Z$ has {\it grouping effect}, then performing spectral 
clustering based on $Z$ would be effective. 
Intuitively, $Z$ has grouping effect if, given two {\it highly correlated} objects $x_i$ and $x_j$,
their characterizations of other objects are similar.
Existing works mostly consider {\it high correlation} between objects as {\it high similarity} of their
feature vectors. With ROSC, we consider object similarity in terms of both feature similarity and 
reachability similarity. 
Feature similarity is measured by the objects' feature vectors as given by the columns of matrix $X$.
Reachability similarity is measured by the columns of matrix $\mathcal{W}$, 
each of which shows the reachability of an object to all others. 
Formally,



%It has been shown that the first two terms in the objective function decide the \emph{grouping effect} of $Z$~\cite{lu2012robust}.
%In Problem~\ref{eq:obj}, the first two terms decides whether $Z$ has the grouping effect~\cite{lu2012robust} defined as follows.
%i.e., the more highly correlated two objects are,
%the larger weight one will have in characterizing the other~\cite{lu2012robust}.

\begin{definition}
\label{def:grouping}
\textbf{(Grouping effect)}. 
Given a set of objects $\mathcal{X} = \{x_1, x_2,..., x_n\}$,
let $\bmw_q$ be the $q$-th column of $\mathcal{W}$. 
Further, let $\xarrow{i}{j}$ denote the condition:
(1) $\bmx_i^T \bmx_j \rightarrow 1$ and 
(2) $\lVert \bmw_i - \bmw_j \rVert_2 \rightarrow 0$.
A matrix $Z$ is said to have grouping effect
if
\[
\xarrow{i}{j} \Rightarrow |Z_{ip} - Z_{jp}| \rightarrow 0\; \forall 1 \leq p \leq n.
\]
%for an arbitrary object $\bmx$ and its associated coefficient vector $\bm{z}$,
%If $\bmx_i\rightarrow \bmx_j$,
%then $z_{pi}\rightarrow z_{pj}$,
%where $z_{pi}$ and $z_{pj}$ are the $i$th and $j$th entry in $\bm{z}_p$ respectively.
%Then we say the self-representation matrix $Z$
%has the grouping effect.
%\hfill$\Box$
\end{definition}

Our next task is to prove that the optimal solution $Z^*$ (as given in Equation~\ref{eq:solution})
% of Equation~\ref{eq:obj_constraint}
has the grouping effect.
In the following discussion, we use $\bmz_q^*$ to denote the $q$-th column vector of $Z^*$.

\begin{lemma}
\label{lemma1}
Given a set of objects $\mathcal{X}$,
the matrix
$X\in \mathcal{R}^{p\times n}$ that is composed of the {\pev}s as rows,
 the reachability matrix $\mathcal{W}$,
 and the optimal soution $Z^*$ of Equation~\ref{eq:obj_constraint},
\begin{equation}
\label{eq:zi}
Z_{ip}^* = \frac{\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*) + \alpha_2 \mathcal{W}_{ip}}{\alpha_1+\alpha_2}, \;\;\; \forall 1 \leq i, p \leq n.
\end{equation}
\end{lemma}

\begin{proof}
For $1 \leq p \leq n$,
let $J(\bm{z}_p) =  ||\bm{x}_p-X\bm{z}_p||_2^2 + \alpha_1 ||\bm{z}_p||_2^2 + \alpha_2 ||\bm{z}_p-\bm{w}_p||_2^2$.
Since $Z^*$ is the optimal solution of Equation~\ref{eq:obj_constraint}, we have $\frac{\partial{J}}{\partial{Z}_{ip}}|_{\bm{z}_p = \bm{z}_p^*} = 0\; \forall 1\leq i \leq n$.
Hence, $-2\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*)+2\alpha_1Z_{ip}^*+2\alpha_2(Z_{ip}^*-\mathcal{W}_{ip}) = 0$,
which induces Equation~\ref{eq:zi}.
\end{proof}

%\begin{lemma}
%\label{lemma1}
%Given a set of objects $X\in \mathcal{R}^{d\times n}$ and a TKNN graph $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathcal{W}_K)$,
%let $\bm{x}_p$ be an arbitrary object and $\bm{w}_p$ be the column vector in $\mathcal{W}_K$ describing the connectivity of $\bmx_p$.
%Each item $z_{pi}^*$ in the optimal solution $\bm{z}_p^*$ to the problem 
%$\min_{\bm{z}} ||\bm{x}_p-X\bm{z}_p||_2^2 + \lambda_1 ||\bm{z}_p||_2^2 + \lambda_2 ||\bm{z}_p-\bm{w}_p||_2^2$ is
%\begin{equation}
%\label{eq:zi}
%z_{pi}^* = \frac{\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*) + \lambda_2 w_{pi}}{\lambda_1+\lambda_2},
%\end{equation}
%where $w_{pi} = 1$, if $\bm{x_p}$ and $\bm{x}_i$ are reachable; $0$, otherwise. 
%
%Proof. Let $J(\bm{z}_p) =  ||\bm{x}_p-X\bm{z}_p||_2^2 + \lambda_1 ||\bm{z}_p||_2^2 + \lambda_2 ||\bm{z}_p-\bm{w}_p||_2^2$.
%Since $\bm{z}_p^*$ is the optimal solution, then $\frac{\partial{J}}{\partial{z}_{pi}}|_{\bm{z}_p = \bm{z}_p^*} = 0$.
%Thus we have $-2\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*)+2\lambda_1z_{pi}^*+2\lambda_2(z_{pi}^*-w_{pi}) = 0$,
%which induces Eq.~\ref{eq:zi}.
%\end{lemma}

\comment{
Eq.~\ref{eq:zi} calculates the weight of object $\bm{x}_i$ in characterizing $\bm{x}$.
For $w_i$, if $\bm{x}$ and $\bm{x}_i$ are reachable in the TKNN graph, $w_i = 1$; otherwise, $w_i = 0$. 
Eq.~\ref{eq:zi} rectifies the ineffective similarity as follows.
When $\bm{x}$ and $\bm{x_i}$ are far away from each other in the feature space
but reachable in the TKNN graph,
$z_i$ will be increased by $w_i = 1$.
%which rectifies the original incorrect similarity value between them.
Moreover, if $\bm{x}$ and $\bm{x}_i$ are highly correlated,
the first two terms in the problem can decide a large $z_i$,
even in the case that they are unreachable.
%$z_i$ can still keep large with a small $\lambda_2$.
In summary, Eq.~\ref{eq:zi} can not only hold the original accurate similarities but also rectify the incorrect ones.

\noindent{\small$\bullet$}
For any two objects dissimilar in the feature space but connected in the TKNN graph, 
their similarity will be increased.

\noindent{\small$\bullet$}
For any two objects dissimilar in the feature space and disconnected in the TKNN graph, 
their similarity will be further decreased.

\noindent{\small$\bullet$}
For any two objects similar in the feature space and connected in the TKNN graph,
their similarity will be further increased.

\noindent{\small$\bullet$}
For any two objects similar in the feature space but disconnected in the TKNN graph,
their similarity will be decreased. In this case,
provided that the raw similarity is effective already,
even though the new value will be decreased,
but it will be still
}

\begin{lemma}
\label{lemma2}
%Given a set of objects $X\in R^{d\times n}$ and a TKNN graph $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathcal{W}_K)$,
%let $\bm{x}_p$ be an arbitrary object, 
%$\bm{w}_p$ be the column vector in $\mathcal{W}_K$ describing the connectivity of $\bm{x}_p$, and
%$\bm{z}_p^*$ be the optimal solution to the problem 
%$\min_{\bm{z}_p} ||\bm{x}_p-X\bm{z}_p||_2^2 + \lambda_1 ||\bm{z}_p||_2^2 + \lambda_2 ||\bm{z}_p-\bm{w}_p||_2^2$.
%Assume all the objects have been normalized.
%For any two objects $\bm{x}_i$ and $\bm{x}_j$,
$\forall 1 \leq i, j, p \leq n$,
\begin{equation}
\label{eq:norm}
|Z_{ip}^*-Z_{jp}^*| \leq \frac{c\sqrt{2(1-r)} + \alpha_2|\mathcal{W}_{ip}-\mathcal{W}_{jp}|}{\alpha_1+\alpha_2},
\end{equation}
where $c = \sqrt{1+\alpha_2||\bm{w}_p||_2^2}$ and $r = \bm{x}_i^T\bm{x}_j$.
\end{lemma}

\begin{proof}
From Equation~\ref{eq:zi}, we have 
\begin{equation}
\nonumber
Z_{ip}^*-Z_{jp}^* = \frac{(\bm{x}_i^T - \bm{x}_j^T)(\bm{x}_p-X\bm{z}_p^*) + \alpha_2 (\mathcal{W}_{ip}-\mathcal{W}_{jp})}{\alpha_1+\alpha_2}.
\end{equation}
That implies 
\begin{small}
\begin{equation}
\label{eq:zizj}
\begin{split}
|Z_{ip}^*-Z_{jp}^*| & \leq \frac{|(\bm{x}_i^T - \bm{x}_j^T)(\bm{x}_p-X\bm{z}_p^*)| + \alpha_2 |\mathcal{W}_{ip}-\mathcal{W}_{jp}|}{\alpha_1+\alpha_2}\\
& \leq \frac{||\bm{x}_i - \bm{x}_j||_2||\bm{x}_p-X\bm{z}_p^*||_2 + \alpha_2 |\mathcal{W}_{ip}-\mathcal{W}_{jp}|}{\alpha_1+\alpha_2}\\
\end{split}
\end{equation}
\end{small}

Since the column vectors of $X$ are normalized (i.e., $\bmx_q^T \bmx_q = 1 \; \forall 1 \leq q \leq n$) , we have
$||\bm{x}_i - \bm{x}_j||_2 = \sqrt{2(1-r)}$,
where $r = \bm{x}_i^T\bm{x}_j$.
%measuring the closeness between $\bm{x}_i$ and $\bm{x}_j$ in the feature space.
%As $\bm{z}_p^*$ is the optimal solution, 
As $Z^*$ is the optimal solution of Equation~\ref{eq:obj_constraint}, we have
\begin{equation}
\begin{split}
J(\bm{z}_p^*) & = ||\bm{x}_p-X\bm{z}_p^*||_2^2 + \alpha_1 ||\bm{z}_p^*||_2^2 + \alpha_2 ||\bm{z}_p^*-\bm{w}_p||_2^2 \leq  \\
J(\bm{0}) & = ||\bm{x}_p||_2^2 + \alpha_2 ||\bm{w}_p||_2^2 = 1 + \alpha_2 ||\bm{w}_p||_2^2.
\end{split}
\end{equation}
Hence, $||\bm{x}_p-X\bm{z}_p^*||_2 \leq \sqrt{1 + \alpha_2 ||\bm{w}_p||_2^2} = c$.
Equation~\ref{eq:zizj} can be further simplified as
\begin{equation}
\nonumber
|Z_{ip}^*-Z_{jp}^*| \leq \frac{c\sqrt{2(1-r)}+ \alpha_2 |\mathcal{W}_{ip}-\mathcal{W}_{jp}|}{\alpha_1+\alpha_2}.
\end{equation}
\end{proof}

\begin{lemma}
Matrix $Z^*$ has grouping effect.
\label{lemma:z-star}
\end{lemma}
\begin{proof}
Given two objects $x_i$ and $x_j$ such that $\xarrow{i}{j}$,
we have,  %by definition, 
(1) $\bmx_i^T \bmx_j \rightarrow 1$ and (2) $||\bmw_{i}-\bmw_{j}||_2 \rightarrow 0$.
These imply
$r = \bmx_i^T \bmx_j \rightarrow 1$ and  $|\mathcal{W}_{ip}-\mathcal{W}_{jp}| \rightarrow 0$.
Hence, the two terms of the numerator of the R.H.S of Equation~\ref{eq:norm} are close to 0. 
Therefore, $|Z_{ip}^*-Z_{jp}^*| \rightarrow 0$ and thus $Z^*$ has grouping effect.
\end{proof}

Indeed, Equation~\ref{eq:norm} shows how our algorithm ROSC enhances the effectiveness of 
spectral clustering on multi-scale data. 
Comparing with traditional approaches, which focus on feature similarity, ROSC uses $Z^*$
to integrate feature similarity  ($r$) with
reachability similarity ($|\mathcal{W}_{ip}-\mathcal{W}_{jp}|$).
In particular, two distant objects $x_i$ and $x_j$ of a cluster may not share a strong feature similarity.
This leads to a small $r$ and traditional approaches will likely put them into separate clusters.
On the contrary, ROSC considers the strong reachability of the objects
to derive a small value of $|\mathcal{W}_{ip}-\mathcal{W}_{jp}|$, and thus keeping them in the same cluster.
Moreover, for $x_i$ and $x_j$ that belong to two different dense clusters but happen to be close in 
space (i.e., $x_i$ and $x_j$ have strong feature similarity), 
traditional approaches may inadvertently merge them into the same cluster. 
ROSC, however, would discover their low reachability (via the mutual-KNN relation)
and derive a large value of $|\mathcal{W}_{ip}-\mathcal{W}_{jp}|$.
This regulates matrix $Z^*$ and avoids the incorrect merging.
As we will see in the next section, ROSC's approach 
greatly improves clustering quality and is more robust than other algorithms in handling
multi-scale data.
 
%Lemma~\ref{lemma1} and~\ref{lemma2} prove the grouping effect of $Z^*$ derived by Eq.~\ref{eq:solution}.
%%the weight difference of two objects in characterizing an arbitrary object $\bm{x}$ is bounded.
%Given two objects $\bmx_i$ and $\bmx_j$, if $\bmx_i \rightarrow \bmx_j$, 
%i.e., $\bmx_i^T \bmx_j \rightarrow 1$ and $||w_{pi}-w_{pj}||_2 \rightarrow 0$,
%then $||z_{pi}^*-z_{pj}^*||_2 \rightarrow 0$.
%%which shows the grouping effect of $Z$ derived by Eq.~\ref{eq:solution}.
%%However, in the case of (1) $\bm{x}_i^T\bm{x}_j = 0$ but $w_i=w_j=1$ and 
%%(2) $\bm{x}_i^T\bm{x}_j = 1$ but $||w_i-w_j||_2=1$,
%%$||z_i^*-z_j^*||_2$ can still be small with an appropriate setting on $\lambda_1$ and $\lambda_2$.
%%Further, since $Z$ can not only retain the accurate similarities but also rectify the incorrect ones, 
%%In other words, objects in the same cluster will be better reflected in the rectified matrix.
%%Such grouping effect together with The rectification ability could guarantee a more robust clustering performance.
%We then summarize how the TKNN graph rectifies the raw similarity matrix.
%Given any two objects $\bmx_i$ and $\bmx_j$,
%\begin{enumerate}[label=(\arabic*), leftmargin=*]
%\setlength{\itemsep}{0pt}
%\setlength{\parsep}{0pt}
%\setlength{\parskip}{0pt}
%\item $\bmx_i^T \bmx_j \rightarrow 0$, $\bmx_i$ and $\bmx_j$ are reachable, the effect of $S_{ij}$ will be increased.
%\item $\bmx_i^T \bmx_j \rightarrow 0$, $\bmx_i$ and $\bmx_j$ are unreachable, the effect of $S_{ij}$ will be further decreased.
%\item $\bmx_i^T \bmx_j \rightarrow 1$, $\bmx_i$ and $\bmx_j$ are reachable, the effect of $S_{ij}$ will be further increased.
%\item $\bmx_i^T \bmx_j \rightarrow 1$, $\bmx_i$ and $\bmx_j$ are unreachable, the effect of $S_{ij}$ will be decreased.
%\end{enumerate}
%Among the four cases,
%$Z$ reserves the efficacy of effective similarities by (2) and (3)
%while it enhances the efficacy of ineffective similarities by (1) and (4). 
%Thus spectral clustering based on $Z$ will be more robust.

\comment{
\noindent{\small$\bullet$}
$\bmx_i^T \bmx_j \rightarrow 0$ but reachable, $S_{ij}$ will be increased.

\noindent{\small$\bullet$}
%For any two objects dissimilar in the feature space and disconnected in the TKNN graph, their similarity will be further decreased.
$\bmx_i^T \bmx_j \rightarrow 0$ and unreachable, $S_{ij}$ will be further decreased.

\noindent{\small$\bullet$}
%For any two objects similar in the feature space and connected in the TKNN graph, their similarity will be further increased.
$\bmx_i^T \bmx_j \rightarrow 1$ and reachable, $S_{ij}$ will be further increased.

\noindent{\small$\bullet$}
$\bmx_i^T \bmx_j \rightarrow 1$ but unreachable, $S_{ij}$ will be decreased.
}

\subsection*{ROSC: Robust Spectral Clustering}
%The coefficient matrix $Z$ take advantage of both cluster-separation information in all the eigenvectors
%and the TkNN graph, which not only retains the original accurate similarities but also rectifies the incorrect ones.

We note that the matrix $Z^*$ obtained may be asymmetric and it may contain negative values.
To construct a matrix of object similarity, a common fix~\cite{liu2013robust,lu2012robust} is to 
compute $\tilde{Z} = (|Z^*|+|(Z^*)^T|)/2$.
After $\tilde{Z}$ is computed, ROSC executes a standard spectral clustering method
(e.g., NCuts) using $\tilde{Z}$ as the similarity matrix in place of $S$.
It can be proved that $|Z^*|$, $|(Z^*)^T|$, and hence $\tilde{Z}$ all have grouping effect.
%Due to space limitations, readers are referred to [XXX] for the proofs. 
Finally, ROSC is summarized in Algorithm~\ref{alg}.

\begin{lemma}
Matrix $|Z^*|$ has grouping effect.
\label{lemma:z-star-abs}
\end{lemma}
\begin{proof}
Given two objects $x_i$ and $x_j$,
we have 
$\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| \leq |Z_{ip}^*-Z_{jp}^*|$.
From Lemma~\ref{lemma:z-star},
$Z^*$ has grouping effect, i.e.,
if $x_i \rightarrow x_j$, $|Z_{ip}^*-Z_{jp}^*| \rightarrow 0$.
Thus $\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| \rightarrow 0$ and 
$|Z^*|$ has grouping effect.
\end{proof}

\begin{lemma}
\label{lemma3}
$(Z^*)^T$ and $|(Z^*)^T|$ have grouping effect. 
\begin{proof}
The problem is equivalent to if $x_i \rightarrow x_j$, $Z^*_{pi} \rightarrow Z^*_{pj}$.
From Lemma~\ref{lemma1},
\begin{equation}
\nonumber
Z_{pi}^*-Z_{pj}^* = \frac{\bm{x}_p^T ( \bmx_i - \bmx_j - X(\bm{z}_i^*-\bm{z}_j^*)) + \alpha_2 (\mathcal{W}_{pi}-\mathcal{W}_{pj})}{\alpha_1+\alpha_2}.
\end{equation}
Since $\bm{z}_i^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_i+\alpha_2\bm{w}_i),\bm{z}_j^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_j+\alpha_2\bm{w}_j)$,
let $Y = X(X^TX + \alpha_1I + \alpha_2I)^{-1}$. Then
\begin{equation}
\begin{split}
|Z_{pi}^*-Z_{pj}^*| & \leq \frac{|\bmx_p^T(\bm{x}_i - \bm{x}_j)| + |\bmx_p^TX(\bm{z}_i^*-\bm{z}_j^*)| + \alpha_2 |(\mathcal{W}_{pi}-\mathcal{W}_{pj})|}{\alpha_1+\alpha_2}\\
& \leq \frac{|\bmx_p^T(\bm{x}_i - \bm{x}_j)| + |\bmx_p^TYX^T(\bmx_i-\bmx_j)|}{\alpha_1+\alpha_2}\\
& + \frac{\alpha_2|\bmx_p^TY(\bm{w}_i - \bm{w}_j)| + \alpha_2 |\mathcal{W}_{pi}-\mathcal{W}_{pj}|}{\alpha_1+\alpha_2}\\
& \leq \frac{||\bmx_p||_2||\bm{x}_i - \bm{x}_j||_2 + ||\bmx_p^TYX^T||_2||\bmx_i-\bmx_j||_2}{\alpha_1+\alpha_2}\\
& + \frac{\alpha_2||\bmx_p^TY||_2||\bm{w}_i - \bm{w}_j||_2 + \alpha_2 |\mathcal{W}_{pi}-\mathcal{W}_{pj}|}{\alpha_1+\alpha_2}\\
\end{split}
\end{equation}
If $x_i \rightarrow x_j$, i.e., $\bmx_i^T\bmx_j \rightarrow 1$ and $||\bm{w}_i - \bm{w}_j||_2 \rightarrow 0$, 
we have
$||\bm{x}_i - \bm{x}_j||_2 \rightarrow 0$ and $|\mathcal{W}_{pi}-\mathcal{W}_{pj}| \rightarrow 0$.
Then $|Z_{pi}^*-Z_{pj}^*| \rightarrow 0$ and
thus $(Z^*)^T$ has grouping effect.
Since $\bigl||Z_{pi}^*|-|Z_{pj}^*|\bigr| \leq |Z_{pi}^*-Z_{pj}^*|$, $|(Z^*)^T|$ also has grouping effect.
\end{proof}
\end{lemma}

\begin{lemma}
\label{lemma4}
Matrix $\tilde{Z}$ has grouping effect. 
\begin{proof}
From Lemma~\ref{lemma:z-star-abs} and~\ref{lemma3},
both $\lvert Z^*\rvert$ and $\lvert (Z^*)^T\rvert$ have the grouping effect.
Since $\tilde{Z} = (|Z^*|+|(Z^*)^T|)/2$,
\begin{equation}
\begin{split}
\lvert \tilde{Z}_{ip} - \tilde{Z}_{jp}\rvert & = \frac{\bigl| (|Z^*_{ip}|+|Z^*_{pi}|) - (|Z^*_{jp}|+|Z^*_{pj}|)\bigr|}{2} \\
& \leq \frac{\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| + \bigl||Z_{pi}^*|-|Z_{pj}^*|\bigr|}{2}
\end{split}
\end{equation}
If $x_i \rightarrow x_j$,
both $\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| \rightarrow 0$ and $\bigl||Z_{pi}^*|-|Z_{pj}^*|\bigr| \rightarrow 0$,
so $\lvert \tilde{Z}_{ip} - \tilde{Z}_{jp}\rvert \rightarrow 0$ and
$\tilde{Z}$ has grouping effect.
\end{proof}
\end{lemma}


\comment{
\begin{lemma}
\label{lemma3}
$(Z^*)^T$ has the grouping effect. 

Proof. The problem is equivalent to if $x_i \rightarrow x_j$, $Z^*_{pi} \rightarrow Z^*_{pj}$.
From Lemma~\ref{lemma1},
\begin{equation}
\nonumber
z_{pi}^*-z_{pj}^* = \frac{\bm{x}_p^T ( \bmx_i - \bmx_j - X(\bm{z}_i^*-\bm{z}_j^*)) + \alpha_2 (W_{pi}-W_{pj})}{\alpha_1+\alpha_2}.
\end{equation}
Since $\bm{z}_i^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_i+\alpha_2\bm{w}_i),\bm{z}_j^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_j+\alpha_2\bm{w}_j)$,
let $Y = X(X^TX + \alpha_1I + \alpha_2I)^{-1}$. Then
\begin{equation}
\begin{split}
||Z_{pi}^*-Z_{pj}^*||_2 & \leq \frac{||\bmx_p^T(\bm{x}_i - \bm{x}_j)||_2 + ||\bmx_p^TX(\bm{z}_i^*-\bm{z}_j^*)||_2 + \alpha_2 ||(W_{pi}-W_{pj})||_2}{\alpha_1+\alpha_2}\\
& \leq \frac{||\bmx_p^T(\bm{x}_i - \bm{x}_j)||_2 + ||\bmx_p^TYX^T(\bmx_i-\bmx_j)||_2}{\alpha_1+\alpha_2}\\
& + \frac{\alpha_2||\bmx_p^TY(\bm{w}_i - \bm{w}_j)||_2 + \alpha_2 ||W_{pi}-W_{pj}||_2}{\alpha_1+\alpha_2}\\
\end{split}
\end{equation}
If $x_i \rightarrow x_j$, i.e., $\bmx_i^T\bmx_j \rightarrow 1$ and $||\bm{w}_i - \bm{w}_j||_2 \rightarrow 0$, 
we have
$||\bm{x}_i - \bm{x}_j||_2 \rightarrow 0$ and $||W_{pi}-W_{pj}||_2 \rightarrow 0$.
Then $||Z_{pi}^*-Z_{pj}^*||_2 \rightarrow 0$,
which proves the grouping effect of $(Z^*)^T$.
%\begin{equation}
%\begin{split}
%||\bmx_p^TX(\bm{z}_i^*-\bm{z}_j^*)||_2 & \leq ||\bmx_p^TY(X^T(\bmx_i-\bmx_j) +\alpha_2(\bm{w}_i - \bm{w}_j))||_2\\
%& \leq ||\bmx_p^TYX^T(\bmx_i-\bmx_j)||_2 +\alpha_2||\bmx_p^TY(\bm{w}_i - \bm{w}_j)||_2\\
%\end{split}
%\end{equation}
\end{lemma}

\begin{lemma}
\label{lemma4}
$\tilde{Z}$ has the grouping effect. 

Proof. From Lemma~\ref{lemma2} and~\ref{lemma3},
both $Z^*$ and $(Z^*)^T$ have the grouping effect,
which can be easily extended to
$|Z^*|$ and $|(Z^*)^T|$.
Since $\tilde{Z} = (|Z^*|+|(Z^*)^T|)/2$,
$\tilde{Z}$ also has the grouping effect.
\end{lemma}

To this end, we summarize ROSC as follows.
ROSC first computes the TKNN graph $\mathcal{G}$
and the associated weight matrix $\mathcal{W}_K$. Then it applies power iteration to generate $p$
pseudo-eigenvectors that form a $p \times n$ matrix $X$.
After whitening and normalization on $X$,
the coefficient matrix $Z^*$ can be calculated by solving Eq.~\ref{eq:solution},
which further leads to the construction of a rectified similarity matrix $\tilde{Z}$.
Since $\tilde{Z}$ has the grouping effect, 
the standard spectral clustering methods (e.g., NCuts) will be finally applied to derive more robust clustering results.
The time complexity of ROSC will be no more than the standard spectral clustering methods,
which is $O(n^3)$ in general.
In the future, we will attempt to improve it. 
}

\begin{algorithm}
\begin{small}
\caption{ROSC}
\label{alg}
\begin{algorithmic}[1]
\Require $S$, $k$.
\Ensure $\mathcal{C} = \{C_1, ..., C_k\}$
\State Compute the TKNN graph and the reachability matrix $\mathcal{W}$
\State Calculate $W = D^{-1}S$, where $D_{ii} = \sum_jS_{ij}$
%\For $j \leftarrow 1$ do
%\State$t = 0$
%\Repeat
%\State $v_j^{t+1} \leftarrow \frac{Wv_j^t}{||Wv_j^t||_1}$
%\State $ \delta^{t+1} \leftarrow |v_j^{t+1} - v_j^t|$
%\State $t$++
%\Until $||\delta_j^t+1 - \delta_j^t||_{max} \leq \epsilon$ or $t\geq T$
%\EndFor
\State Apply PI on $W$ and generate $p$ pseudo-eigenvectors $\{\bm{v}_r\}_{r=1}^p$
\State $X = \{\bm{v}_1^T; \bm{v}_2^T; ...; \bm{v}_p^T\}$; $X$ = whiten($X$)
\State Normalize each column vector $\bm{x}$ of $X$ such that $\bm{x}^T\bm{x} = 1$
\State Calculate the coefficient matrix $Z^*$ by Eq.~\ref{eq:solution}
\State Construct $\tilde{Z} = (|Z^*| + |(Z^*)^T|)/2$
\State Run standard spectral clustering methods, e.g., NCuts, with $\tilde{Z}$ as the
similarity matrix to obtain clusters $\mathcal{C} = \{C_r\}_{r=1}^k$
%\State Decode $\{C_r\}_{r=1}^k$ from $\{{\bm z_r}\}_{r=1}^k$
\State \Return $\mathcal{C} = \{C_1, ..., C_k\}$
\end{algorithmic}
\end{small}
\end{algorithm}









==> tex/optimization.tex <==
\subsection{Model optimization}
\label{sec:optimization}

Our objective is to find the best clustering, or equivalently, the indicator vectors $\{\bm{z}_r\}_{r=1}^k$ that 
minimizes the penalty function $\mathcal{J}()$.
Note that $\mathcal{J}()$ is a function of $\bml$ and $\bmo$ (which are the weights of meta-paths and object
attributes), whose values need to be learned as well.
\schain\ learns these parameters using an iterative mutual update approach. 
Each iteration consists of two steps. First, given $\bml$ and $\bmo$, we find the optimal clustering 
$\{\bm{z}_r\}_{r=1}^k$. Second, given $\{\bm{z}_r\}_{r=1}^k$, we
find the optimal $\bml$ and $\bmo$.
\schain\ iterates until the change in the penalty is smaller than a threshold $\epsilon$ or 
a fixed number of iterations have been executed.
Next, we show how the two update steps are performed.

\subsubsection{Finding the optimal $\{${\boldmath $z$}$_r\}_{r=1}^k$ given {\boldmath $\lambda$} and \boldmath $\omega$}

For fixed values of $\bml$ and $\bmo$, $\mathcal{J}()$ is a function of $\bmz$.
We define a matrix $\tilde{Z}$, where its $r$-th column
$\tilde{Z}_{\cdot r}$ 
equals $D^{\frac{1}{2}}\bm{z}_r/(\bm{z}_r^TD\bm{z}_r)^{\frac{1}{2}}$. 
Note that since $\tilde{Z}^T\tilde{Z} = I_k$, where $I_k$ is the $k \times k$ identity matrix,
$\tilde{Z}$ is an orthonormal matrix.
For fixed values of $\bml$ and $\bmo$, minimizing $\mathcal{J}()$ is equivalent to minimizing:
%\begin{small}
\begin{equation}
\label{eq:obj:trans2}
\begin{split}
\mathcal{J}'(\tilde{Z}) & = \mathit{trace}(\tilde{Z}^TD^{-\frac{1}{2}}(D-S-W\circ S)D^{-\frac{1}{2}}\tilde{Z}), \\
%& = \mathit{trace}(\tilde{Z}^TD^{-\frac{1}{2}}DD^{-\frac{1}{2}}\tilde{Z}-\tilde{Z}^TD^{-\frac{1}{2}}(S+ W\circ S)D^{-\frac{1}{2}}\tilde{Z}) \\
& = \mathit{trace}(I_k-\tilde{Z}^TD^{-\frac{1}{2}}(S+W\circ S)D^{-\frac{1}{2}}\tilde{Z}).
\end{split}
\end{equation}
%\end{small}
Since $trace(I_k)$ is a constant, the above is equivalent to solving the following trace maximization problem:
\begin{equation}
\begin{split}
\label{eq:max}
& \max_{\tilde{Z}^T\tilde{Z} = I_k}\mathit{trace}(\tilde{Z}^TD^{-\frac{1}{2}}(S+W\circ S)D^{-\frac{1}{2}}\tilde{Z}).  \\
\end{split}
\end{equation}
Since $\tilde{Z}$ is a rigorous cluster indicator matrix, the optimization problem is NP-hard~\cite{DBLP:dblp_conf/icml/LongZWY06}.
To address this issue, we allow real relaxation to $\tilde{Z}$ so that its entries can assume real values. Then,
according to the Ky-Fan theorem~\cite{bhatia1997matrix}, 
the maximization problem (\ref{eq:max}) has a closed-form solution that corresponds to the subspace spanned 
by the top $k$ eigenvectors of $K = D^{-\frac{1}{2}}(S+W\circ S)D^{-\frac{1}{2}}$. 
Since $\tilde{Z}_{\cdot r} = D^{\frac{1}{2}}\bm{z}_r/(\bm{z}_r^TD\bm{z}_r)^{\frac{1}{2}}$,
we need to transform each $\tilde{Z}_{\cdot r}$ back to a real-relaxed $\bm z_r$. 
We first calculate
$U = D^{-\frac{1}{2}}\tilde{Z}$ and then
normalize it by column.
Each column in $U$ is a real-relaxed $\bm z_r$.
Finally, with the real relaxation, entries in $U$ take on fractional values, so the clustering is not
definite. To derive a hard clustering, 
we treat each row in $U$ as a feature vector of an object.
After row normalization on $U$, we adopt $k$-means to cluster objects.
%a postprocessing step is required and we adopt $k$-means to convert $\tilde{Z}$ to $\{\bm {z}_r\}_{r=1}^k$.
%we take the cluster membership values of each object (derivable from $\bmz$)
%as features of objects and cluster the objects using $k$-means based on these cluster membership features.

\subsubsection{Finding the optimal {\boldmath $\lambda$} and {\boldmath $\omega$} given $\{${\boldmath $z$}$_r\}_{r=1}^k$}
%After clusters are derived, they can be used to supervise the weight learning of meta paths and attributes, 
%because different meta paths and attributes play different roles in determining the formation of these clusters.
%Therefore, we can optimize $\bm \lambda$ and $\bm \omega$ based on the results of $\{\bm z_i\}_{i=1}^k$.

For fixed $\{\bm z_r\}_{r=1}^k$, $\mathcal{J}()$ is a function of $\bml$ and $\bmo$.
We rewrite Eq.~\ref{eq:obj:trans:reg} as:
\begin{small}
\begin{equation}
\label{eq:obj:trans3}
\begin{split}
\mathcal{J}(\bm \lambda, \bm \omega) & = 
%\sum_{i=1}^k\frac{\bm{z}_i^T(D-S- \mathcal{W} \circ S)\bm{z}_i}{\bm{z}_i^TD\bm{z}_i} + \gamma(||\bm\lambda||^2+||\bm \omega||^2) \\
%& = 
\sum_{r=1}^k\frac{\bm{z}_r^TD\bm{z}_r-\bm{z}_r^T(S+ \mathcal{W} \circ S)\bm{z}_r}{\bm{z}_r^TD\bm{z}_r} + \gamma(||\bm\lambda||^2+||\bm \omega||^2), \\
& = k - \sum_{r=1}^k\frac{\bm{z}_r^T(S+ \mathcal{W} \circ S)\bm{z}_r}{\bm{z}_r^TD\bm{z}_r} + \gamma(||\bm\lambda||^2+||\bm \omega||^2). \\
%& + \gamma(\|\bm \lambda\|^2 + \sum_{c=1}^k \|A_c\|_F^2),
\end{split}
\end{equation}
\end{small}
Since $k$ is a constant, minimizing $\mathcal{J}(\bml, \bmo)$ is equivalent to maximizing:
\begin{equation}
\label{eq:obj:trans4}
%\mathcal{J}''(\bml, \bmo) = 
\max_{\bm \lambda, \bm \omega} \sum_{r=1}^k\frac{\bm{z}_r^T(S+ \mathcal{W} \circ S)\bm{z}_r}{\bm{z}_r^TD\bm{z}_r}
- \gamma(||\bm \lambda||^2+||\bm \omega||^2).
\end{equation}
Note that the entries of matrices $S$ and $D$ are linear functions of $\bml$ and $\bmo$.
Therefore, the numerator and the denominator of each term in the summation are both linear functions of $\bml$ and $\bmo$.
Hence, (\ref{eq:obj:trans4})
can be rewritten as:
%can be reformulated to a nonlinear polynomial fractional programming (NPFP) problem~\cite{dinkelbach1967nonlinear}.

%\textbf{Nonlinear polynomial fractional programming problem (NPFPP)}.
%$f(\bm \lambda, \{A_i\}_{i=1}^k) = \sum_{u=1}^p a_u\prod_{j = 1}^{|\mathcal{PS}|}(\lambda_j)^{b_u}\prod_{i=1}^k\prod_{j=1}^{|\mathcal{A}|}((A_i)_{jj})^{c_{uij}}$, 
%$g(\bm \lambda, \{A_i\}_{i=1}^k) = \sum_{u=1}^q r_u \prod_{j = 1}^{|\mathcal{PS}|}(\lambda_j)^{s_u}\prod_{i=1}^k\prod_{j=1}^{|\mathcal{A}|}((A_i)_{jj})^{t_{uij}}$.
%Then Eq.~\ref{eq:obj:trans4} can be revised as
\begin{equation}
\label{eq:obj:trans5}
\mathcal{H}(\bml, \bmo) = \max_{\bm \lambda, \bm \omega} \frac{f(\bm \lambda, \bm \omega)}{g(\bm \lambda, \bm \omega)},
\end{equation}
where
$f(\bm \lambda, \bm \omega)$ and $g(\bm \lambda, \bm \omega)$ are two nonlinear multivariate polynomial functions.

It is shown in~\cite{dinkelbach1967nonlinear} that the maximization problem with the form shown in Eq.~\ref{eq:obj:trans5} can be solved by solving the following
related {\it non-linear parametric programming} problem:
%It is difficult to directly perform analysis on a NPFP problem to determine the existence of solution, so it is necessary to 
%convert this kind of problem into an easy-to-solve one. 
%
%\begin{theorem}
%\label{theo:NPFP}~\cite{DBLP:dblp_journals/jgo/TuyTK04}
%The above NPFP problem is equivalent to the following polynomial programming (PP) problem
%\begin{equation}
%\label{eq:obj:trans6}
%\max_{\bm \lambda, \bm \omega, \eta} \eta f(\bm \lambda, \bm\omega)
%\end{equation}
%subject to $\sum_{i=1}^{|\mathcal{PS}|}\lambda_i = 1$,$\lambda_i \geq 0$, $i = 1,2,...|\mathcal{PS}|$,
%$\sum_{j=1}^{|A|}\omega_j = 1$, $\omega_j \geq 0$, $j = 1,2,...|A|$
%and $0 \leq \eta \leq 1/g(\bm \lambda, \bm \omega)$.
%\comment{
%Proof: Suppose $(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k, \hat \eta)$ is an optimal solution for Eq.~\ref{eq:obj:trans6},
%obviously, $\hat \eta = 1/g(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$ and $\hat \eta f(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k) = 
%f(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)/g(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$. Then for any solution $(\bm \lambda, \{A_i\}_{i=1}^k)$ for NFPP,
%setting $\eta = 1/g(\bm \lambda, \{A_i\}_{i=1}^k)$ satisfies the constraints for PPPPC. Since $(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k, \hat \eta)$
%corresponds to the maximum value of Eq.~\ref{eq:obj:trans6}, we have $\eta f(\bm \lambda, \{A_i\}_{i=1}^k) \leq \hat \eta f(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$
%, i.e., 
%$f(\bm \lambda, \{A_i\}_{i=1}^k)/g(\bm \lambda, \{A_i\}_{i=1}^k) \leq$ $f(\hat{\bm \lambda},$ $\{\hat A_i\}_{i=1}^k)$$/g(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$.
%Therefore, $(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$ solves NFPP.
%
%Conversely, suppose $(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$ solves NFPP. Then for any solution $(\bm \lambda, \{A_i\}_{i=1}^k, \eta)$ for PPPPC, 
%we have $\eta f(\bm \lambda, \{A_i\}_{i=1}^k)$ $\leq f(\bm \lambda, \{A_i\}_{i=1}^k)/g(\bm \lambda, \{A_i\}_{i=1}^k) \leq f(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)/g(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$. By setting $\hat \eta = 1/g(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$, obviously, $(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k, \hat \eta)$ solves PPPPC.
%}
%\hfill$\Box$
%\end{theorem}
%
%According to Theorem~\ref{theo:NPFP}, the NPFP problem can be solved by 
%solving an equivalent PP problem at the cost of adding one more parameter.
%Obviously, the added parameter brings in new burden and is not preferred.
%Moreover, it is well known that the key to solving a global optimization problem is to transcend an incumbent value of the objective function,
%so we can reformulate the NPFP problem into a nonlinear parametric programming (NPP) problem and further simplify it.
%Using the same symbols in Eq.~\ref{eq:obj:trans5}, we define
\begin{definition}
\label{def:npp}
\textbf{[Non-linear parametric programming (NPP)]}
Let $f(\bml,\bmo)$ and $g(\bml,\bmo)$ be two multivariate polynomial functions. For a given $\mu$, find
\begin{equation}
\label{eq:obj:trans7}
F(\mu) = \max_{\bm \lambda, \bm \omega} \left( f(\bm \lambda, \bm \omega) - \mu g(\bm \lambda, \bm \omega) \right).
\end{equation}
In our context, the parameters $\bml$ and $\bmo$ are subject to the constraints listed at the end of Section~\ref{sec:penalty}.
%subject to $\sum_{i=1}^{|\mathcal{PS}|}\lambda_i = 1$,$\lambda_i \geq 0$, $i = 1,2,...|\mathcal{PS}|$ and
%$\sum_{j=1}^{|A|}\omega_j \newline= 1$, $\omega_j \geq 0$, $j = 1,2,...|A|$.
\hfill$\Box$
\end{definition}
In~\cite{dinkelbach1967nonlinear}, the following theorem is proved.
\begin{theorem}
\label{theorem2}
Given a fixed $\mu$, let $({\bm \lambda^*}, {\bm \omega^*})$ be the optimal solution to $F(\mu)$ (Eq.~\ref{eq:obj:trans7}).
$(\bm \lambda^*, \bm \omega^*)$ is also an optimal solution to $\mathcal{H}(\bml, \bmo)$ (Eq.~\ref{eq:obj:trans5}) if and only if $F(\mu) = 0$.
%$f(\bm \lambda, \{A_i\}_{i=1}^k) = \sum_{u=1}^p a_u \prod_{j = 1}^{|\mathcal{PS}|}(\lambda_j)^{b_u}\prod_{i=1}^k$ $\prod_{j=1}^{|\mathcal{A}|}((A_i)_{jj})^{c_{uij}}$, 
%$g(\bm \lambda, \{A_i\}_{i=1}^k) = \sum_{u=1}^q r_u \prod_{j = 1}^{|\mathcal{PS}|}(\lambda_j)^{s_u}\prod_{i=1}^k$ $\prod_{j=1}^{|\mathcal{A}|}((A_i)_{jj})^{t_{uij}}$.
\hfill$\Box$
\end{theorem}

Besides Theorem~\ref{theorem2}, a few lemmas are also proved in~\cite{dinkelbach1967nonlinear}:
%Theorem~\ref{theorem2} reduces the NPFP problem to a NPP problem \emph{in the same parameter space},
%which is much simpler compared with PP problem. Also it is much easier to solve a NPP problem than a NPFP problem.
%Besides, we have some lemmas to help with the optimization.

\begin{lemma}
\label{lemma1}
$F(\mu)$ is convex.
\comment{
Proof: Suppose $(\bm \lambda, \{A_i\}_{i=1}^k)$ is the solution corresponding to $\mu = t\mu_1 + (1-t)\mu_2$,
where $\mu_1 \neq \mu_2, 0 \leq t \leq 1$. Then we have $F(\mu) = f(\bm \lambda, \{A_i\}_{i=1}^k) - \mu g(\bm \lambda, \{A_i\}_{i=1}^k)
= f(\bm \lambda, \{A_i\}_{i=1}^k) - (t\mu_1 + (1-t)\mu_2)g(\bm \lambda, \{A_i\}_{i=1}^k) = t(f(\bm \lambda, \{A_i\}_{i=1}^k) - \mu_1g(\bm \lambda, \{A_i\}_{i=1}^k))
+ (1-t)(f(\bm \lambda, \{A_i\}_{i=1}^k) - \mu_2g(\bm \lambda, \{A_i\}_{i=1}^k))$.
Obviously, $f(\bm \lambda, \{A_i\}_{i=1}^k) - \mu_1g(\bm \lambda, \{A_i\}_{i=1}^k) \leq F(\mu_1)$ and 
$f(\bm \lambda, \{A_i\}_{i=1}^k) - \mu_2g(\bm \lambda, \{A_i\}_{i=1}^k) \leq F(\mu_2)$,
which induces $F(t\mu_1 + (1-t)\mu_2) \leq tF(\mu_1)+(1-t)F(\mu_2)$.
}
\hfill$\Box$
\end{lemma}
\begin{lemma}
\label{lemma2}
$F(\mu)$ is continuous.
\hfill$\Box$
\end{lemma}
\begin{lemma}
\label{lemma3}
$F(\mu)$ is strictly monotonically decreasing, i.e., if $\mu_1 < \mu_2$, $F(\mu_1) > F(\mu_2)$.
\comment{
Proof: Suppose $(\hat{\bm \lambda}, \{\hat{A}_i\}_{i=1}^k)$ is the solution corresponding to $\mu_2$. 
Then we have $F(\mu_2) = f(\hat{\bm \lambda}, \{\hat{A}_i\}_{i=1}^k) - \mu_2g(\hat{\bm \lambda}, \{\hat{A}_i\}_{i=1}^k) 
< f(\hat{\bm \lambda}, \{\hat{A}_i\}_{i=1}^k) - \mu_1g(\hat{\bm \lambda}, \{\hat{A}_i\}_{i=1}^k) \leq 
\max_{\bm \lambda, \{A_i\}_{i=1}^k} f(\bm \lambda, \{A_i\}_{i=1}^k) - \mu_1 g(\bm \lambda, \{A_i\}_{i=1}^k) = F(\mu_1)$
}
\hfill$\Box$
\end{lemma}
\begin{lemma}
\label{lemma4}
$F(\mu) = 0$ has a unique solution.
\hfill$\Box$
\end{lemma}
Due to space limit, 
readers are referred to~\cite{dinkelbach1967nonlinear, stancu2012fractional} for the proofs of the theorem and lemmas.

From Theorem~\ref{theorem2}, we need to find
a $\mu^*$ and its corresponding $({\bm \lambda^*}, {\bm \omega^*})$ such that $F(\mu^*) = 0$.
\schain\ does so by an iterative numerical method.
In each iteration, \schain\ computes a $\mu$ and $(\bml, \bmo)$.
Let $\mu_i$, $(\bml_i, \bmo_i)$ be those computed in the $i$-th iteration.
\schain\ first sets $\mu_1 = 0$ and in each iteration, performs two steps:
(Step 1:) Solve the NPP problem (Eq.~\ref{eq:obj:trans7}) for $\mu = \mu_i$ and set $(\bml_i, \bmo_i)$ to be the solution found. 
(Step 2:) Set $\mu_{i+1} = f(\bml_i, \bmo_i)/g(\bml_i, \bmo_i)$.
Next, we show theoretical properties of this update process.

\noindent{\bf Property 1:}
$\bm{F(\mu_1) > 0}$. 
Without loss of generality, we assume $f(\bml, \bmo) > 0$ and $g(\bml, \bmo) > 0$.\footnote{One can show that the quantity (\ref{eq:obj:trans4})
is bounded below by $-2\gamma$. We can add an arbitrary large constant to (\ref{eq:obj:trans4}) to make it, and thus 
$f(\bml, \bmo)$ and $g(\bml, \bmo)$, positive.}
Now, $F(\mu_1)$ = $F(0)$ = $\max_{\bml, \bmo} f(\bm \lambda, \bm \omega) > 0$.

\noindent{\bf Property 2: if} $\bm{F(\mu_i) > 0}$ {\bf then} 
$\bm {0 \leq F(\mu_{i+1}) < F(\mu_i)}$.
Since $(\bml_i, \bmo_i)$ is the solution of the NPP problem for $\mu = \mu_i$ (Eq. \ref{eq:obj:trans7}),
we have $f(\bml_i, \bmo_i) - \mu_i g(\bml_i, \bmo_i) = F(\mu_i) > 0$.
Hence, $\mu_{i+1} = f(\bml_i, \bmo_i)/g(\bml_i, \bmo_i) > \mu_i$.
By Lemma~\ref{lemma3}, $F(\mu_{i+1}) < F(\mu_i)$.
Also, we have
$F(\mu_{i+1})$ = $\max_{\bm \lambda, \bm \omega} ( f(\bm \lambda, \bm \omega) -\mu_{i+1}g(\bm \lambda, \bm \omega))
\geq f(\bm \lambda_i, \bm \omega_i) - \mu_{i+1} g(\bm \lambda_i, \bm \omega_i) = 0$.

From the properties, we see that \schain\ starts with a positive $F(\mu)$, whose value 
stays positive and decreases across iterations until it reaches 0.
The update procedure thus converges to the optimal values.
%The process is repeated until a certain maximum number of iterations have been executed, or until $F(\mu_i)$ becomes
%negative for some iteration $i$. 
%In the latter case, due to Lemma~\ref{lemma3}, we know that $\mu^* \in [\mu_{i-1}, \mu_i]$.
%\schain\ then switches to the bisection method:
%It computes $\mu_{i+1} = (\mu_{i-1} + \mu_i)/2$, and repeats either with the interval $[\mu_{i-1}, \mu_{i+1}]$ or $[\mu_{i+1}, \mu_i]$,
%depending on which interval contains $\mu^*$. 
The \schain\ algorithm is summarized in Algorithm~\ref{alg}.
\begin{algorithm}
\begin{small}
\caption{SCHAIN}
\label{alg}
\begin{algorithmic}[1]
%\Require $G=(V, E)$, $A$, meta-paths $\mathcal{P}$'s, $\mathcal{X}_i$, $\mathcal{L}$, $D$, $B$, $N_s$.
\Require $G$, $\mathcal{M}$, $\mathcal{C}$, $T_i$, $k$, $\mathcal{PS}$.
\Ensure $\mathfrak{C} = \{C_1, ..., C_k\}$
\State Compute similarity matrices $S_A$, $S_L$, and $S$
\State $t=0$, $\Delta \mathcal{J} = \infty$
%\State Derive $S$ by Eq.~\ref{eq:S}
\State $\bm \lambda = (\frac{1}{|\mathcal{PS}|}, ..., \frac{1}{|\mathcal{PS}|})$;
$\bm \omega = (\frac{1}{|A_i|}, ..., \frac{1}{|A_i|})$
%\State Calculate $\mathit{QS}(D)$
\While{$\Delta \mathcal{J} > \epsilon$ or $t$ < max\_iter}
%\State Construct $\mathcal{M}$ and $\mathcal{C}$
\LeftComment Step 1: Optimize $\{\bm z_r\}_{r=1}^k$ given {$\bm \lambda$} and $\bm \omega$
\State Solve Eq.~\ref{eq:max} to obtain real-relaxed $\tilde{Z}$
\State Calculate $U=D^{-1/2}\tilde{Z}$ and normalize it
\State Derive $\{{\bm z}_r\}_{r=1}^k$ from $U$ by k-means
\LeftComment Step 2: Optimize {$\bm \lambda$} and $\bm \omega$ given $\{${$\bm z$}$_r\}_{r=1}^k$
\State $j=1$; $\mu_j = 0$
%\For{$j = 0$ to $F(\mu)$ converges to 0}
\Repeat
\State Solve Eq.~\ref{eq:obj:trans7} with $\mu = \mu_j$ to obtain ${\bm \lambda}_{j}$, ${\bm \omega}_{j}$
\State $\mu_{j+1} = f({\bm \lambda}_{j}, {\bm \omega}_{j}) / g({\bm \lambda}_{j}, {\bm \omega}_{j})$; $j$++
\Until  $F(\mu_{j+1})$ converges to 0%($j$ > max\_iter2) %or ($F(\mu_j) < 0$) 
%\If{($F(\mu_j) < 0$)}
%\State use bisection method to determine $\bml$, $\bmo$
%\Else 
%\State $\bml = \bml_j$; $\bmo = \bmo_j$
%\EndIf
\State $\Delta \mathcal{J}$ = change in $\mathcal{J}$ with the updated $\{{\bm z_r}\}_{r=1}^k$, $\bml$, $\bmo$
\State $t$++
%\State $\bm \lambda^{t+1} = \hat{\bm \lambda}^{j+1}$; $\bm \omega^{t+1} = \hat{\bm \omega}^{j+1}$
\EndWhile
\State Decode $\{C_r\}_{r=1}^k$ from $\{{\bm z_r}\}_{r=1}^k$
\State \Return $\mathfrak{C} = \{C_1, ..., C_k\}$
\end{algorithmic}
\end{small}
\end{algorithm}






\comment{

In conclusion, to solve a NPFP problem, we need to first convert it into a NPP problem. 
To solve the NPP problem, it involves in two steps. The first step is to select a $\mu$ value and the second one is to solve the maximization problem in
Eq.~\ref{eq:obj:trans7} to get $(\bm \lambda, \bm \omega)$ and $F(\mu)$.
Since the final aim is to find the $\mu$ which makes $F(\mu) = 0$,
we adopt an iterative two-step update strategy to perform optimization.
Step 1: given a $\mu$, solve the maximization problem in Eq.~\ref{eq:obj:trans7} to get $(\bm \lambda, \bm \omega)$ and the $F(\mu)$ value.
Step 2: given $(\bm \lambda, \bm \omega)$, calculate a new $\mu$ value.
Due to the monotonically decreasing property of $F(\mu)$,
we can start from a $\mu$ which makes $F(\mu) > 0$. 
%and $F(0) = \max_{\bm \lambda, \bm \omega} f(\bm \lambda, \bm \omega) > 0$, 
%we can start from $\mu = 0$. 
After $(\bm \lambda, \bm \omega)$ is calculated, according to Proposition~\ref{prop1}, we assign $\mu = f(\bm \lambda, \bm \omega)/g(\bm \lambda, \bm \omega)$.
The iteration repeats until $F(\mu) = 0$.

Since $||\bm \lambda||^2 \leq 1$ and $||\bm \omega||^2 \leq 1$,
we usually add a term $2\gamma$ to the end of Eq.~\ref{eq:obj:trans4} 
to ensure $-\gamma(||\bm \lambda|| ^ 2 + ||\bm \omega||^2) + 2\gamma \geq 0$.
On the one hand, the added term is irrelevant to $\bm \lambda$ and $\bm \omega$,
so it will not influence the optimization result.
On the other hand, it can ensure the derived $f(\bm \lambda, \bm \omega) > 0$ in Eq.~\ref{eq:obj:trans5}.
Since $F(0) = \max f(\bm \lambda, \bm \omega) > 0$,
we can safely start from $\mu = 0$.


\begin{proposition}
\label{prop1}
Suppose $F(\hat \mu) > 0$ and $(\hat{\bm \lambda}, \hat{\bm \omega})$ solves Eq.~\ref{eq:obj:trans7} corresponding to $\hat \mu$, 
then $f(\hat{\bm \lambda}, \hat{\bm \omega})/g(\hat{\bm \lambda}, \hat{\bm \omega}) > \hat \mu$.

Proof: $F(\hat \mu) = \max_{\bm \lambda, \bm \omega} f(\bm \lambda, \bm \omega) - \hat \mu g(\bm \lambda, \bm \omega) =
f(\hat{\bm \lambda}, \hat{\bm \omega}) - \hat \mu g(\hat{\bm \lambda}, \hat{\bm \omega}) > 0$.
$g$ derives from Eq.~\ref{eq:obj:trans4}, as the denominator,
$g(\hat{\bm \lambda}, \hat{\bm \omega}) > 0$,
so we have $f(\hat{\bm \lambda}, \hat{\bm \omega})/g(\hat{\bm \lambda}, \hat{\bm \omega}) > \hat \mu$.
\hfill$\Box$
\end{proposition}

Based on the above iterative optimization method, the model will finally converge.
Proofs are listed as follows.
\begin{theorem}
\label{theorem3}
The proposed model finally converges.

Proof: The objective is to minimize Eq.~\ref{eq:obj:trans:reg}, which includes three parts.
First, $0 \leq \bm{z}_i^T(D-S)\bm{z}_i / \bm{z}_i^TD\bm{z}_i \leq 1$.
Second, for $-(\bm{z}_i^TW\circ S\bm{z}_i / \bm{z}_i^TD\bm{z}_i)$, we consider two extreme cases:
if all the object pairs in cluster $i$ are in the must-link set $\mathcal{M}$, then $0 \leq \bm{z}_i^TW\circ S\bm{z}_i / \bm{z}_i^TD\bm{z}_i \leq 1$;
if all the object pairs in cluster $i$ are in the cannot-link set $\mathcal{C}$, then $-1 \leq \bm{z}_i^TW\circ S\bm{z}_i / \bm{z}_i^TD\bm{z}_i \leq 0$,
so $-1 \leq \bm{z}_i^TW\circ S\bm{z}_i / \bm{z}_i^TD\bm{z}_i \leq 1$, i.e., $-1 \leq -(\bm{z}_i^TW\circ S\bm{z}_i / \bm{z}_i^TD\bm{z}_i) \leq 1$.
Third, since $\gamma \geq 0$, $\gamma (||\bm \lambda||^2 + ||\bm \omega||^2)$ is convex, the constraints on $\bm \lambda$ and $\bm \omega$ are 
also convex, so  
%$\sum_{i=1}^{|\mathcal{PS}|}\lambda_i = 1$, $\sum_{i=1}^{|\mathcal{PS}|}\lambda_i = 1$,$\lambda_i \geq 0$ and $\lambda_j \geq 0$,
it must have a minimum value.
In conclusion, Eq.~\ref{eq:obj:trans:reg} has a lower bound.

Furthermore, the iterative optimization method, either optimizing $\{${\boldmath $z$}$_i\}_{i=1}^k$ or 
updating $\bm \lambda$ and $\bm \omega$, always decreases the objective function, so the convergence is guaranteed.
\hfill$\Box$
\end{theorem}

}









==> tex/preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}
%\subsection{Spectral clustering}
\comment{
Given a set of objects $\mathcal{X} = \{x_1,x_2,...,x_n\}$,
spectral clustering first constructs an undirected graph with $S$ as the similarity (affinity) matrix.
Depending on the different partition strategies,
two main classes of approaches have been suggested.
One class of spectral clustering methods employ the second eigenvector
of the (normalized) graph Laplacian to partition the graph into two subgraphs and 
recursively partition the subgraphs until $k$ partitions~\cite{shi2000normalized}.
It has been shown that cuts based on the second eigenvector give a guaranteed approximation to the optimal cut~\cite{chung1997spectral}.
The second class of methods directly perform $k$-way partition.
They perform eigen-decomposition on the normalized graph Laplacian
(or on the normalized similarity matrix)
to map objects into low-dimension embeddings
by the $k$ smallest eigenvectors (or the $k$ largest eigenvectors).
Taking these eigenvectors as feature vectors of objects,
a standard clustering algorithm like k-means will be applied to return clusters.
%$G = (V,E,S)$ with $V = \mathcal{X}$, $E = \{e_{ij}\}$ and $S = \{s_{ij}\}$,
%where $e_{ij}$ is an edge between objects $x_i$ and $x_j$ with
%weight $s_{ij}$ representing the similarity between them.
%The weight can be calculated in the beginning of spectral clustering or directly given.
It has been experimentally shown that more eigenvectors will be better~\cite{alpert1995spectral,malik2001contour},
so we study the second class in this paper.
}

Spectral clustering is a well-studied topic.
For an introduction and an analysis of the method, see~\cite{von2007tutorial,ng2001spectral,kannan2004clusterings}.
%Figure~\ref{figure:flow_graph}(a) shows the basic pipeline of spectral clustering. 
There are a number of variants of the basic method, some of which differ in the 
way they normalize the graph Laplacian,
$D-S$, where $D$ is the diagonal matrix with $D_{ii} = \sum_j S_{ij}$.
For example, the \emph{normalized cuts} (NCuts) method~\cite{shi2000normalized} 
employs random-walk-based normalization $D^{-1}(D-S)$
while the \emph{Ng-Jordan-Weiss} (NJW) method~\cite{ng2001spectral}  uses symmetric normalization $D^{-\frac{1}{2}}(D-S)D^{-\frac{1}{2}}$.

There are many previous works studying the various aspects of spectral clustering techniques.
For example, there are studies
that focus on the performance of spectral clustering under different data characteristics~\cite{huang2009spectral, von2008consistency, zhu2014constructing},
on computational efficiency~\cite{cheng2003recursive,
chen2011large,cullum2002lanczos,gittens2013approximate,yan2009fast,dhillon2007weighted},
and on the probabilistic theory of the method~\cite{meila2001random,nadler2005diffusion,lafon2006diffusion}.

%Spectral clustering transforms clustering into a graph partition problem. 
%The standard spectral clustering methods vary in the normalization type.
%For example, the \emph{normalized cuts} (NCuts)~\cite{shi2000normalized} method
%employs random walk based normalization $D^{-1}(D-S)$
%while the \emph{Ng-Jordan-Weiss} (NJW)~\cite{ng2001spectral} method uses symmetric normalization $D^{-\frac{1}{2}}(D-S)D^{-\frac{1}{2}}$,
%where $D$ is the diagonal matrix with $D_{ii} = \sum_j S_{ij}$ 
%and $D-S$ is the graph Laplacian.
%%Method without any normalization also exists.
%In this paper, the calculation of the similarity matrix $S$ is out of our concern and $S$ will be given as input.
%We take NJW as an example and summarize
%the pseudocode in Algorithm~\ref{alg1}.
%\begin{algorithm}
%\begin{small}
%\caption{NJW}
%\label{alg1}
%\begin{algorithmic}[1]
%\Require $S$, $k$.
%\Ensure $\mathfrak{C} = \{C_1, ..., C_k\}$
%\State Calculate a diagonal matrix $D$ with diagonal elements: 
%
%$D_{ii} = \sum_{j=1}^n{S_{ij}}, i=1,2,...,n$
%\State Calculate the normalized Laplacian matrix: 
%
%$L = D^{-\frac{1}{2}}(D-S)D^{-\frac{1}{2}}$
%\State Calculate the $k$ smallest eigenvectors of $L$
%\State Perform k-means on the eigenvectors and derive $\mathfrak{C}$
%\State \Return $\mathfrak{C} = \{C_1, ..., C_k\}$
%\end{algorithmic}
%\end{small}
%\end{algorithm}


%Instead of explicit eigen-decomposition of a matrix,
%PIC is competent in reducing the cost 
%by a number of matrix-vector multiplications.

\comment{
\subsection{Definition}
\begin{definition}
\textbf{Distance-based similarity}. Given two objects $\bmx_i,\bmx_j \in R^d$,
the distance-based similarity measures their affinity based on the feature distance.
The measure should be symmetric and non-negative.
\hfill$\Box$
\end{definition}

\begin{example}
Gaussian kernel is a common choice, which has been widely used in spectral clustering. 
Given two objects $\bmx_i,\bmx_j$, 
$S_{ij} = exp(-\frac{||\bmx_i-\bmx_j||^2}{2\sigma^2})$,
where $||\cdot||$ denotes the standard Euclidean distance
and $\sigma$ is the scaling parameter.
\end{example}

\comment{
When the data contains multi-scale clusters,
there may not be a single value of $\sigma$ that works well for all the data.
In~\cite{zelnik2004self}, a measure considering local scaling is introduced.
}

\begin{example}
In the case of multi-scale clusters,
~\cite{zelnik2004self} calculates  
$S_{ij} = exp(-\frac{||\bmx_i-\bmx_j||^2}{\sigma_i\sigma_j})$,
where $\sigma_i,\sigma_j$ denote the local scaling parameters for objects $\bmx_i,\bmx_j$ respectively.
The local scaling parameters adjust the similarity between $\bmx_i$ and $\bmx_j$
according to local statistics of their neighborhoods.
\end{example}

Generally, the similarity between objects in the same cluster should be large 
while the similarity between objects in different clusters should be small. 
However, in the case of multi-scale data,
the distance-based similarity is likely to be abnormal.

\begin{definition}
\textbf{effective/Ineffective similarity}. 
Given two objects $\bmx_i$ and $\bmx_j$,
$S_{ij}$ is an effective similarity
if (1) $S_{ij}$ is large and $L(\bmx_i) = L(\bmx_j)$
or (2) $S_{ij}$ is small and $L(\bmx_i) \neq L(\bmx_j)$,
where $L(\cdot)$ denotes the true cluster label function.
Otherwise, $S_{ij}$ is an ineffective similarity
if (1) $S_{ij}$ is large but $L(\bmx_i) \neq L(\bmx_j)$
or (2) $S_{ij}$ is small but $L(\bmx_i) = L(\bmx_j)$.
\hfill$\Box$
\end{definition}

\begin{example}
In Fig.~\ref{figure:example1},
$S_{34}$ is an effective similarity because $\bmx_3$ and $\bmx_4$ belong to the same cluster 
and $S_{34}$ is large due to the short distance.
However, $S_{23}$ is an ineffective similarity because $\bmx_2$ and $\bmx_3$
have the same cluster label but they are far away from each other, leading to a small $S_{23}$.
Further, $S_{12}$ is also an ineffective similarity as $\bmx_1$ and $\bmx_2$ are in different clusters but with high similarity.
\end{example}
}









